Network Backbone Discovery Using Edge Clustering

In this paper, we investigate the problem of network backbone discovery. In complex systems, a "backbone" takes a central role in carrying out the system functionality and carries the bulk of system traffic. It also both simplifies and highlight underlying networking structure. Here, we propose an integrated graph theoretical and information theoretical network backbone model. We develop an efficient mining algorithm based on Kullback-Leibler divergence optimization procedure and maximal weight connected subgraph discovery procedure. A detailed experimental evaluation demonstrates both the effectiveness and efficiency of our approach. The case studies in the real world domain further illustrates the usefulness of the discovered network backbones.

==> Backbone.tex <==
\section{Network Backbone Discovery}
\label{backbone}

%\subsubsection{Background and Basic Idea}
%\label{background}
%\vspace*{-2.0ex}

In many man-made complex systems, a ``backbone'' takes a central role in carrying out the system functionality. The
clearest examples are the highway framework in the transportation system and the backbone of the Internet. When
studying these systems, the backbone offers both a concise and highlighted view. Interestingly, the backbone phenomena
has recently been observed in several natural and social systems, including metabolic networks~\cite{CN:Almass04},
social networks~\cite{CN:Kossinets08}, and food webs~\cite{SgelesSerrano04212009}. Clearly, discovering and extracting
network backbones is essential in understanding the organization principle of complex systems and a key step towards
``map'' functionality in complex network analysis. Unfortunately, there is no formal definition of the network
backbone. All the existing work merely captures the backbone as whatever their particular heuristic procedures find.

\begin{figure*}

    \centering
    \mbox{
        \subfigure[Network and its backbone]{\includegraphics[width=1.5in,height=1.2in]{Figures/backbone.eps}\label{f1}}
    }
    \mbox{
        \subfigure[Coding of subgraph]{\includegraphics[width=1.5in,height=1.2in]{Figures/graphcoding1.eps}\label{f2}}
    }
    \mbox{
        \subfigure[Path coding example]{\includegraphics[width=1.5in,height=1.2in]{Figures/pathcoding.eps}\label{f3}}
    }

    \caption{Path encoding with and without backbone}

        \label{fig:graphcode}
\end{figure*}


\comment{
However, all of the existing research rely additional information, such as communication and temporal information to identify the backbone, and most importantly,  there is no any formal definition of the network backbone.
Most of the complex networks do not have such information.
More importantly, there is no any formal definition of the network backbone.
All existing studies utilize some heuristic procedures to define and extract the backbone.}

We propose an integrated graph theoretical and information theoretical framework to model the network backbone.
Intuitively, the network backbone is a connected subgraph which carries major network ``traffic''.
% and enables fast ``information flow''.
%Where does the traffic come from in the complex network?
A complex system's behavior relies on the proper communication/coordination through the underlying network substrate,
which invokes a sequence of local interactions between adjacent pair of vertices.
These interactions thus form system-wide network traffic ~\cite{CN:Rosvall08b}.
It is essential for a complex system to deliver such traffic in an energy efficient way~\cite{BaddiP99}.
Here, at least two energy costs need to be considered:
1) the communication cost and 2) the organization cost in defining/recognizing the communication path.
For the first cost, the energy efficient way for one vertex communicating with another vertex naturally points to the shortest path.
%In the complex network, each edge may associate with a weight to describe the cost of its corresponding local interaction.
The second cost can be described as a path-recognition complexity.
Based on information theory, we could depict it as the shortest coding length of a given path.
%In Figure~\ref{}, we show a path description using its edge sequence..
%Then, each edge is assigned with a unique code.
In general, the optimal code length for an edge $(i,j)$ can be bounded by $\log \frac{1}{p(i\rightarrow j)}$, where $p(i\rightarrow j)$ is the probability of a shortest path taking edge $(i,j)$ when it goes through  vertex $i$~\cite{CoverThomas91}.

% i.e., out of all the shortest paths going through vertex $i$, the fraction of them directly connecting to vertex $j$~\cite{}.
%Indeed, we note that a slightly different formulation of the second cost has been applied for community detection in complex network~\cite{}.

Minimizing these two costs gives rise to the network backbone structure: the shortest paths form a traffic flow which must efficiently travel from source to destination using the backbone.  A backbone that is too simple or has the wrong topology is not an efficient route for all vertex-vertex paths (first cost).  A backbone that is too complex is expensive to describe (second cost).
This clearly complies with our intuition of a backbone structure.
%Figure~\ref{} illustrates a backbone and its usage in reducing the description length of a shortest path.
Figure~\ref{fig:graphcode} illustrates a backbone and its usage in reducing the description length of a shortest path. Huffman code is used here only for illustrative purpose. The proposed computational framework does not rely on a particular coding scheme.
Figure~\ref{f1} shows a network with its highlighted backbone.
Figure \ref{f2} shows the Huffman code for each edge in the subgraph, where upper part is for the edge code without
utilizing backbone and lower part is for using backbone.
For instance, the edge $(9,2)$ with direction $9 \rightarrow 2$ is assigned with code $1$, and with direction $2 \rightarrow 9$ is assigned with code $000$ in the upper part example.
In Figure~\ref{f3}, we show a path coding using and without using the backbone.
We basically list each edge code in the path consecutively.
Specifically, the subpath $(2,3,4,5)$ is in the backbone, and we use ``['' and ``]'' to denote the entering and exiting of the backbone, respectively.
Note that even with an extra coding cost of entering and exiting from the backbone, the lower coding cost of paths inside the backbone can still be beneficial.




\subsection{Problem Formulation and Proposed Approach}
\label{formulaation}


\bdefin{\bf (Network Backbone Problem)}
\label{backboneproblem}
Given complex network $G=(V,E)$, the network backbone $B=(V_B,E_B)$ is a connected subgraph, such that $\sum_{(u,v) \in V\times V} w(u,v) \times {C(P(u,v))}$ is minimal, where $P(u,v)$ is the shortest path from vertex $u$ to $v$, $C(P(u,v))$ is its coding cost, and $w(u,v)$ is its communication frequency.
\edefin
Without any prior knowledge, $w(u,v)$ has equal weight.
In many systems, this weight can be estimated.

Clearly, the exact solution of this problem is very computationally expensive.
Even computing the optimal score of a given backbone $\sum {w(u,v) \times C(P(u,v))}$ is costly.
We propose to utilize a weighted second-order graph to help approximate a relative score (coding savings) due to the backbone.
Further, a novel ``core-growth-prune'' strategy can be employed on top of the second-order graph to discover the network backbone.
The overall algorithm can be described in three major steps (illustrated in Figure~\ref{fig:alg1}).


\noindent{\bf Step 1 (Construction Weighted Second-Order Graph):}
We will first transform the original network into its {\em second-order} counterpart, $G^\prime$, by converting each edge in $G$ into a edge-vertex and two edge-vertices are adjacent if they share a common vertex in $G$.
Figure~\ref{fig:alg1}(a) shows the converted second-order graph from Figure~\ref{fig:graphcode}(a).
The introduction of the second-order graph allows us to represent and compute an approximate overall coding saving by a backbone efficiently.
Specifically, the second-order graph is weighted: each edge-vertex in the second order graph is associated with two values $\delta_1(e)$ and $N_1(e)$, and
each edge $(e_1,e_2)$ is associated with $\delta_2(e_1,e_2)$ and $N_2(e_1,e_2)$.
Both $\delta_1$ and $\delta_2$ are zero for the non-backbone edges.
Intuitively, for an edge-vertex $e_b$, $\delta_1(e_b)<0$ records a penalty for its isolated occurrence in any shortest path (no other backbone edges come before or after it). This is because of the extra coding cost for entering and exiting from the backbone.
For edge $(e_1,e_2)$, $\delta(e_1,e_2)>0$ records the coding saving by their consecutive occurrence in a shortest path.
Further, $N_1(e)$ and $N_2(e_1,e_2)$ record the number of isolated occurrence for any backbone edge $e$, and the total number of shortest paths which contain consecutive $e_1$ and $e_2$, respectively.
Given this, our goal can be transformed to {\em identification of an induced subgraph in $G^\prime=(V_B^\prime,E_B^\prime)$ in the second order graph,
such that
$\sum_{e \in V_B^\prime} N_1(e) \times \delta_1(e)+ \sum_{(e_1,e_2) \in E_B^\prime}
N_2(e_1,e_2) \times \delta_2(e_1,e_2)$  is maximized}.
%Here, $V_B^\prime$ is the vertex-edge set of the backbone and $E_B^\prime$ is the edge set of the backbone in the second order subgraph.
Since this criteria considers only the savings for consecutive backbone edges in any shortest path, it serves as a lower bound of the total coding savings.

\begin{figure*}[t!]
    \centering
    \mbox{
        \subfigure[$Second-order$ graph and its initial core]{\includegraphics[width=1.5in,height=1.3in]{Figures/initsg.eps}\label{s1}}
    }
    \mbox{
        \subfigure[Expanded core]{\includegraphics[width=1.5in,height=1.3in]{Figures/growsg.eps}\label{s2}}
    }
    \mbox{
        \subfigure[Extracted backbone]{\includegraphics[width=1.5in,height=1.3in]{Figures/extractedbackbone.eps}\label{s3}}
    }

    \caption{Backbone extraction example}
    \label{fig:alg1}

\end{figure*}


\noindent{\bf Step 2 (Backbone Core Discovery):} Once we have the weighted second order graph, $G^\prime$, the second
step is to identify a group of edge vertices which can form a core for the backbone. Starting from this core, we can
grow the complete backbone. The difficulty of this step is that we do not have any penalty/saving value $\delta_1$ and
$\delta_2$ since there is no backbone at this point. To simplify the problem, penalty/saving value $\delta_1$ and
$\delta_2$ can be viewed as input parameters specified by users (actually, one parameter $\frac{\delta_1}{\delta_2}$ is
enough if we fix $\delta_2$ as 1). Intuitively, backbone emerges from original network structure such that network
itself can serve as the candidate of backbone. Here, we assume initial backbone is the original network and compute the
values of $N_1$ and $N_2$. Given this, the problem is converted to finding a connected subgraph which maximize the cost
$\sum_{e \in V_B^\prime} N_1(e) \times \delta_1(e)+ \sum_{(e_1,e_2) \in E_B^\prime} N_2(e_1,e_2) \times
\delta_2(e_1,e_2)$. Note that, $V_B^\prime$ is $V$ and $E_B^\prime$ is $E$ at initial point. Our problem is superficially
similar to classical maximal connected subgraph \cite{Li09}. The most remarkable different is we are working on the
graph with weights on both vertices and edges instead of only vertex-weight or edge-weight graph for maximal connected
subgraph. The heaviest subgraph, pruned to improve the overall coding score,  will serve as the core of the backbone.
The highlighted subgraph in Figure \ref{s1} illustrates the initial core.

\comment{Once we have the weighted second order graph, $G^\prime$, the second step is to identify a group of edge vertices which can form a core for the backbone. Starting from this core, we can grow the complete backbone.
The difficulty of this step is that we do not have any penalty/saving value $\delta_1$ and $\delta_2$ since there is no backbone at this point.
The number of isolated backbone edge $N_1$ is also zero.
Thus, the only information available is the weight $N(e_1,e_2)$ associated with each edge in the second order graph.
Figure~\ref{fig:alg1}(a) shows the edge weight $N(e_1,e_2)$ higher than $10$.
Given this, a good starting point seems to be an induced subgraph whose average number of two consecutive edges in the shortest paths per edge
$\frac{\sum_{(e_1,e_2) \in E_B^\prime} N_2(e_1,e_2)}{|V_B^\prime|}$ is maximal.
This corresponds to the {\em weighted densest subgraph} problem.
The fastest exact algorithm for this problem runs in $O(|V||E| \log {|V|^2/|E|})$ ~\cite{GGT89} using a maximal flow technique.
An efficient approximation algorithm has also been proposed ~\cite{Charikar00}.
The densest induced subgraph, pruned to improve the overall coding score,  will serve as the core of the backbone.
The highlighted subgraph in Figure \ref{s1} illustrates the initial core.
}


\noindent{\bf Step 3 (Backbone Growth and Pruning):}
In the final step, we will {\em iteratively refine} the network backbone by adding new edge vertices to it until there is no further improvement of the goodness score.
To facilitate this iterative refinement step, a priority queue is established by associating a score for each candidate backbone edge-vertex.
The score is based on an estimated savings each can offer.
The estimated savings of a candidate edge-vertex will be revised when any of its adjacent edge-vertex is added in the backbone.
The growing step will be finished when all the estimated savings become negative.
Finally, we perform an edge pruning of the identified subgraph to improve the coding efficiency. The result is our final backbone.
Figure~\ref{s2} and ~\ref{s3} show the final backbone in the second order graph and in the original network, respectively.
%Figure~\ref{s3} highlights the extracted backbone in the original network.
The numbers associated with the edges in Figure~\ref{s3} are the corresponding edge-vertices in the second-order graph in Figure~\ref{s2}.



\subsection{Research Issues to be Investigated}
\label{issue}

\noindent{\bf Scalability:} How to extract the backbone from a large complex network is a challenging issue. As we
discussed earlier, in the proposed algorithm, we either need to compute the pair-wise shortest path or pair-wise
transition matrix. This is prohibitive for a large network. We plan to apply a sampling technique for this problem. For
the deterministic case, we can sample a limited number of vertices and computing their shortest path to all other
vertices. We will use these shortest paths to extract backbones. For the random shortest path, we will extract some
long distance shortest pairs and use them to extract backbones. This is because the backbone mainly facilitates
long-range communication. Another technique we will explore is utilizing the relationship between modularity and
backbone. This is based on the observation that between-module edges are likely to become part of the network backbone.
We will investigate how to systematically select and integrate those edges into the backbone.

\noindent{\bf Backbone Validation:} We plan to validate the backbone in two contexts. In the first context, we will use
a transportation network, the Internet, or other network with a known backbone structure to see how many edges/nodes
can be discovered by our backbone extraction problem. Second, we plan to extract and study network backbones from
biological networks and social networks. In biological networks, we will try to understand the biological meaning of
the backbone, by analyzing them under different biological conditions. In social networks, we plan to analyze how the
backbone affects the communication structure. Also, we will study the {\em robustness} of backbones in terms of
edge/vertex changes, and how sensitive they are with respect to parameters in the randomized shortest path model.


\noindent{\bf Backbone Application:} As discussed in the last section, one of my research focuses is on developing
indices to answer distance queries or reachability queries on large graphs. A network backbone provides a tool for
capturing the major traffic along the shortest path connections. We plan to investigate how to apply the backbone
structure to build indices for answering distance queries on large graphs. A particular angle we will explore is how to
constrain the backbone to be a tree-shape and how this backbone-tree can be used in indexing.


==> Backbone_new.tex <==
\subsection{Information Backbone Discovery}
\label{backbone}

A key open question in system biology is how cellular systems are organized for support their adaptive and even intelligent behavior. The existing research focuses on the static structure of biological networks and the {\em network modularity} has been discovered as a fundamental organization principle of cellular system~\cite{citeulike:302050,16916470,citeulike:239}. 
Modularity suggests that more interactions exist between nodes within the same module and less interactions between inter-module nodes. 
A number of network clustering methods have been developed to 
decompose a complex network into densely connected (or functionally homogeneous) components, thus revealing 
reveal such modularity-structure ~\cite{Newman03,Newman04m,CN:Handcock07,CN:Hastings06,CN:Karrer08,CN:Rosvall08a}.

However, modularity does not model how network is organized to enable the global (inter-modular) communication. In many man-made complex systems, a ``backbone'' takes a central role in carrying out the system functionality. Examples of network backbone structure include the highway framework in the transportation system and the backbone of the Internet. 
Interestingly, the backbone phenomena has recently been observed in several natural and social systems, including metabolic networks~\cite{CN:Almass04}, multi-tissue co-expression network~\cite{19463160}, social networks~\cite{CN:Kossinets08}, and food webs~\cite{SgelesSerrano04212009}.
Clearly, discovering and extracting network backbones is essential in understanding the organization principle of biological systems. 
Unfortunately, there is no formal definition of the network backbone. 
All the existing work merely captures the backbone as whatever their particular heuristic procedures find.

\comment{
\begin{figure*}

    \centering
    \mbox{
        \subfigure[Backbone and information flows]{\includegraphics[width=1.5in,height=1.2in]{Figures/inforbackbone.eps}\label{ff1}}
    }
    \mbox{
        \subfigure[Coding of subgraph without backbone]{\includegraphics[width=1.5in,height=1.2in]{Figures/graphcode.eps}\label{ff2}}
    }
    \mbox{
        \subfigure[Coding of subgraph with backbone]{\includegraphics[width=1.5in,height=1.2in]{Figures/graphcodebb.eps}\label{ff3}}
    }

    \caption{Graph encoding with and with backbone}
        \label{fig:graphcode}

\end{figure*}
\textcolor{red}{New Backbone Discovery Algorithm}}

\subsubsection{The Concept of Information Backbone}
\label{probdef}
Intuitively, the information backbone is a connected and sparse subgraph which carries major network "traffic" (information flow).
It can simplify and highlight the underlying structures and the traffic flows in the complex network.
A complex system's behavior relies on the proper communication/coordination through the underlying network substrate,
which invokes a sequence of local interactions between adjacent pair of vertices.
These interactions thus form system-wide network traffic ~\cite{CN:Rosvall08b}.
Especially as a complex system always tends to deliver such traffic in an energy efficient way~\cite{BaddiP99}, the information flow from one vertex to another over a network naturally follows the shortest paths~\cite{GirvanNewman02}. 
Given this, the traffic each edge carries can be measured in terms of {\em edge betweenness}~\cite{GirvanNewman02}, i.e., the number of shortest paths between pairs of vertices that pass through it. 
Thus, a connected subgraph which is composed of high betweenness edges (``carries'' major short-path traffic flow) emerges into the backbone of the underlying network. 

Formally, let $G=(V,E)$ be the network (protein-protein interaction network in this project) with edges $E \subseteq V \times V$ and let $\mathcal{P}$ be the collection of paths in network $G$ which corresponds to the communication channel carrying the system flow.
With no prior knowledge, we consider $\mathcal{P}$ to contain the shortest paths for each pair of vertices in graph $G$, i.e, $\mathcal{P}=\cup P_{uv} $, where $P_{uv}$ records all the shortest paths between $u$ and $v$.
In addition, let $P_{uv}(e)$ records all the shortest paths between $u$ and $v$ which contains edge $e$. 
Given this, the betweenness of edge $e$, $b(e)$, is defined as 
%\beqnarr
$b(e)=\sum_{u,v \in V \times V} \frac{|P_{uv}(e)|}{|P_{uv}|}$. 
%\eeqnarr 
Efficient algorithms are available to compute the edge betweenness for a  large network~\cite{Brandes01afaster,brandes08on}. 

Given graph $G=(V,E)$ and the edge betweenness measure $b(e)$ for each edge $e \in E$, we would like to find a connected subgraph which can best capture our intuition on the information backbone, i.e., carrying the major information flow. 
Two main factors should be both taken into consideration for measuring the ``goodness'' of a connected subgraph serving as the information backbone: 1) the overall edge betweenness in the subgraph and 2) the complexity and especially the size of the subgraph. 
The importance of the second factor is that it can help avoid the over-complex backbone and also allow us to study backbone at different scales. Putting these factors together, the information discovery problem can be defined as follows: 

\bdefin{\bf (Information Backbone Discovery Problem)}
Given a complex network $G=(V,E)$ and the edge betweenness measure $w(e)$ for each edge $e \in E$ with respect to the targeted path set $\mathcal{P}$, 
we define the information backbone $B=(V_B,E_B)$ to be a connected subgraph
such that $L \le |E_B| \le U$ and $\frac{\sum_{e \in E_B} w(e)}{|E_B|}$ is maximized,
where $L$ and $U$ are lower and upper bound of the number of edges in the backbone. 
\edefin

We also refer to this problem as the {\em dense betweenness subgraph} problem since the ``goodness'' of a candidate backbone subgraph is measured in terms of its average edge betweenness instead of the overall betweenness. 
This can naturally take the second factor (backbone size) into consideration. 
However, such a goodness function introduces a trap: without the size factor, 
the best backbone is a single-edge subgraph which contains the highest edge betweenness. 
The lower bound parameter $L$ can help avoid this trap. 
The purpose of the upper bound parameter $U$ is in two folds: 
first, combining with $L$, they would allow user to 
specify the desired the backbone size, and second it can help 
to reduce the search space. 

\subsubsection{An Efficient Approach for Backbone Discovery}
Finding the optimal backbone is closely related to the NP-hard {\em maximum edge-weight connected subgraph} problem~\cite{Li09,Yamamoto09,Lee98,Lee96} which search for an $k$ edge connected subgraph with maximum sum of edge weights $\sum w(e)$. In the meantime, it is computationally prohibitive to enumerate all the connected subgraphs between $L$ and $U$ for identifying the optimal information backbone. 

To efficiently discover the backbone subgraph in a given large graph, we propose a two stage approach, which consists of a ``seed-growth'' step to produce a candidate backbone, and a ``pruning'' step to discover the desired backbone structure. 

\noindent{\bf (Step 1) Betweenness Flooding Algorithms for Candidate Backbone Generation:}
Let us start with the ideal situation where the backbone can be easily determined: 
Assuming the edges are ordered based on their edge betweenness, if the top-$L$ edges actually form a connected subgraph, then this subgraph is the optimal backbone. 
However, in the general situation, these top betweenness edges may not directly link with one another. 
As indicated in ~\cite{GirvanNewman02}, they tend to appear between the components, i.e., 
the shortest-paths communication from one component to another utilizes those between-component edges. 
This is similar to transportation system as the highway often serves as the link between two areas, such as cities or states.  
Given this, we can see that the major problem of the backbone discovery is how to extend and connect those top betweenness edges to form the backbone subgraphs. 

Specifically, we propose an efficient ``betweenness flooding'' procedure to discover the candidate backbone, which is likely to contain the optimal backbone as a subgraph. 
The basic idea is to start with the top $L$ betweenness edges and they will ``flood'' their adjacent edges following the order of betweenness. The higher betweenness edge will be flooded first. This flooding process will be stopped until the top $L$ betweenness edges are connected or certain size constraint is reached. 

\noindent{\bf (Step 2) Greedy Backbone Refinement:}
In this stage, for each connected component generated in the first step, we will identify its maximal betweenness subgraph (the candidate backbone) and choose the best one among these candidate backbones. 
Different from the earlier ``growing'' stage, this stage only considers 
the removal of edges so that the number of edges in the candidate backbone would satisfy the size constraint ($L$ and $U$). 
It is not hard to see that this problem is indeed equivalent to the original backbone discovery problem on a smaller scale, i.e., on the connected component detected in the first stage,  not on the entire network. 
What being unique here is that each connected component serves as the substrate to link those highest betweenness edges and this resembles the resulting backbone.
Our goal is to remove those edges which are not essential to such connection, i.e., edges have low betweenness and removal it does not affect the connectivity. 
The straightforward way to achieve this is through a greedy refinement procedure: in each step of the procedure, we ensure there is only one connected component after the edge removal. 
Specifically, we greedily {\em choose the edge which has the lowest edge betweenness whose removal will not result in disconnecting the remaining vertices in the component.}
We iteratively perform the edge removal until the number of edges in the components reach the lower bound. 
The subgraph between $L$ and $U$ which has the highest average betweenness will be selected as our candidate backbone. 


\subsubsection{Preliminary Backbone Discovery}
We applied the backbone discovery algorithm on the human protein-protein interaction (PPI) dataset obtained from ~\cite{HumanPPI05} to identify backbone of the human PPI. The algorithm returned the genes in the backbone with the user specified size (which is 200 in our test). As shown in Figure~\ref{fig:NetVis}, the backbone genes contain many well known and important genes in cellular signaling transduction pathways including both kinases (e.g., {\em RAF1}, {\em MAPK14}, {\em SRC} and {\em FYN}) and receptors (e.g., {\em TRAF6}, {\em PDGFRB}) as well as signaling molecules such as {\em PDGFB}. Unlike traditional gene set discovery studies for which we expect to obtain a group of genes with a small set of specifically enriched functions or pathways, we expect that the backbones genes of the PPI network would be engaged in many different functions and possibly pathways. The functional and pathway analysis using tools such as the Ingenuity Pathway Analysis (IPA) indeed confirmed our expectation. As shown in Figure \ref{fig:IPA}, the 200 genes are highly enriched with a wide spectrum of important biological functions and are related to many different diseases with high statistical significance. Moreover, they are involved in a large number of pathways, which is very rare for a gene list of this size. For the IPA canonical pathways, the 200 genes show enrichment with p-values (of the Fisher's exact test used by IPA) less than 0.0001 for more than 70 different pathways. These observations suggest that many backbone genes may involve in more than one pathways.  Indeed we found that out of the 200 genes (of which 195 can be mapped to KEGG gene ids) 47 are involved in at least {\em four} KEGG pathways. This is a highly significant enrichment comparing to the fact that a total 1,100 such genes can be found among the entire genome of 19,076 annotated human genes in the KEGG database ($p < 1.9\times 10^{-17}$ for hypergeometric test). It can be conceived that perturbation on these genes can lead to serious disruption of important biological functions, which implies the involvement in diseases in human. This is also confirmed as shown in Figure~\ref{fig:IPA}. Therefore, our preliminary study on the PPI network backbone discovery demonstrated the effectiveness of our approach and its great potential as a new gene ranking tool.

However, since the PPI networks obtained from existing databases usually do not contain condition specific information and they do not provide the functional characterization of the networks such as the amount of information. It is the purpose of this proposal to further extend the backbone discovery to specific tissues and conditions and integrate the information flow with backbone discovery using gene expression data and PPI network data.

\begin{figure*}
    \centering
    \mbox{
        \includegraphics[height=1.8in, width=5.0in]{Figures/NetworkVis.epsi}
%, bb=0 0 1417 519
    }

    \caption{Visualization of the 200 gene backbone for the PPI network.  Red color indicates genes involving in at least 4 KEGG pathways. The larger the nodes, the more KEGG pathways they are involved in.}
        \label{fig:NetVis}

\end{figure*}

\begin{figure*}
    \centering{
    \includegraphics[height=1.5in, width=2.0in]{Figures/Picture1.epsi}\label{IPA1}
%, bb=0 0 791 664
    \includegraphics[height=1.5in, width=2.0in]{Figures/Picture3.epsi}\label{IPA3}
%, bb=0 0 889 664
    \includegraphics[height=1.5in, width=2.0in]{Figures/Picture2.epsi}\label{IPA2}
%, bb=0 0 681 664
    }

    \caption{Function and pathway enrichment analysis on the 200 backbone genes by IPA. Left: Top 15 enriched functional categories. Middle: Top 15 enriched canonical pathways. Right: Top 15 diseases and disorders.}
        \label{fig:IPA}

\end{figure*}

\subsubsection{Biological Implications and Applications of Information Backbone}
The concept of information backbone provides a new perspective on characterizing the functions of the network. With the current interactome or gene co-expression network, we cannot immediate infer important pathways besides results from the network topology analysis such as hub genes. However, once the information flow is overlaid on such networks, the connections between genes can be ranked and the backbones may highly correlate with the robustness of the network functions. Just like a breakdown of major interstate highway may cause significant influence on the traffic at the national scale while the block of a local road only has limited effects on the traffic, the perturbation on the backbone may cause significant loss of function on the gene network. Thus while the mutation of a hub gene often leads to  significant structure and topology change in a gene network, the effects of the blockade of the network backbone is on the functional level. To verify this notion, we will apply the algorithms to both the fruitfly neural degeneration project and the mouse tissue network project. By identifying the network backbones in these samples under different conditions, we can understand the biological meaning of the backbone. 

In addition, we will investigate how information backbone and modularity coexists and how they affect each other.  It seems that the backbone emerges as the long distance information path, while the modularity comes from the fact that a lot of communication takes in local places. There have been little study on how they  work together. We plan to analyze the backbone structure and the modularity structure on the biological network and social network and empirically study their relationship. 




%2) we will apply the {\em weighted densest subgraph} algorithm~\cite{} in $G^\prime$ to identify a proper core for the network backbone; 
%3) we will {\em iteratively refine} the network backbone by adding new edge vertices to the backbone until no further improvement of a goodness score. 



\comment{To facilitate this iterative refinement step, a priority queue is established by associating a score to each candidate backbone edge-vertex. 
The final backbone is a local optimal induced subgraph in the second order graph $G^\prime$.} 

\comment{

%\vspace*{-3.0ex}
\subsubsection{Generalization using Randomized information  path}
%\vspace*{-2.0ex}
We will investigate relaxing the information  path constraint for pair-wise vertex communication. This is based on the observation that an absolute information  path may be replaced with a slightly longer path but with lower cost of recognition, and certain randomness may be involved in the information cascading in situations like congestion. 
We plan to utilize the recently proposed random information  path model~\cite{YenSMS08} for this purpose. 
This model provides a unified framework to capture those nondeterministic factors, and also generalizes both the deterministic information  path and the natural random walk~\cite{DoyleSnell00}. 
Specifically, for any communication from $u$ to $v$, we will specify a ``path-walking'' matrix (transition probability matrix), which determines at each given vertex, what is the transition probability in going to its neighbors.
At high level, there can be a collection of paths from $u$ to $v$, denoted as $R(u,v)$, where each of them associated with a path probability $p(r), r \in R(u,v)$.
In the random information  path, the path probability is defined through the transition probability matrix. 
In particular, given two vertices $u$ and $v$, we can find the transition probability matrix which can minimize the expected path length $\sum_{r \in R_{(u,v)}} p(r) |r|$, where $|r|$ is the path length, subject to a fixed relative entropy ({\em Kullback-Leibler divergence}) with respect to the natural random walk, $\sum_{r\in R(u,v)}{p(r) \log \frac{p(r)}{p^n(r)}} =J_0$, where $p^n(r)$ is the path probability using natural random walk and $J_0$ is the fixed relative entropy. If $J_0$ is $0$, we have the natural random walk, and when $J_0$ increases, the paths probability distribution is centered around the information  path. 



\comment{As an example, suppose we will just take the information  path from vertex $u$ to $v$ and let the path be $(v_0,v_1,\cdots,v_k)$, where $u=v_0$ and $v_k=v$. 
Then, the transition  probability matrix $T$ has $T[v_{i-1},v_{i}]=1$ $1 \leq i \leq k$, where other cells are zero. 
If we consider the natural random walk, then the transition probability matrix is defined by $T[u,v]=\frac{1}{d(u)}$ if $u$ and $v$ is adjacent. Otherwise $T[u,v]=0$. 
Basically, at each vertex, we randomly choose walking to its neighbor.

Given two vertices $u$ and $v$, we would like to find the transition  probability matrix to minimize the expected path length from $u$ to $v$ subject to a fixed relative entropy ({\em Kullback-Leibler divergence}) with respect to the natural random walk: 
\[ \min{ \sum_{r \in R_{(u,v)}} p(r) D(r) } \mbox{  subject to  }
\sum_{r\in R(u,v)}{p(r) \log \frac{p(r)}{p^n(r)}} =J_0\]
Here $J_0$ is a used specified priori (if $J_0$ is $0$, we have the natural random walk, and when $J_0$ increases, the paths probability distribution is centered around the information  path) ; $R(u,v)$ is the all the possible paths from $u$ to $v$ including cycles; $p(r)$ is the probability of this path $r$ is being taken under the transition probability matrix; $p^n(r)$ is the path probability using typical random walk; and $D(r)$ is the path length.
An efficient linear algebra approach is developed to find the optimal transition probability matrix~\cite{}. }

Under the randomized information  path model, our backbone problem can be formulated as follows:  {\em given complex network $G$, the network backbone $B=(V_B,E_B)$ is a connected subgraph, such that $\sum_{(u,v) \in V \times V} w(u,v) \times 
\sum_{r \in R(u,v)} C(r)p(r)$ is minimized}.
Note that the major difference from this problem to the original problem (Definition~\ref{backboneproblem}) is that each path is reweighed accordingly to a path probability.  

To solve this problem, we can factor in the path probability for the coding cost.
%we note that the main difference is that we have to consider the path probability for the coding cost. 
%If we factor in the path probability,
Then, the proposed algorithm for the original backbone extraction problem can be directly applied here. 
However, this would require computing the transition matrix for every ($u$,$v$) pair. 
This is much more expensive than finding only the information  path.  
We will discuss this issue in the next subsection. 

\comment{We basically need rewrite the saving of a path $r_{(u,v)}$ as $w(u,v)\times p(r_{(u,v)})$. 
This can be further factored into the savings of every connective backbone edges. 
What we need to do is instead of computing $N_1$ and $N_2$ using the number of information  path, but for each pair $u$ and $v$, computing the expected number of paths contain them, or contain such isolated occurrence.
The rest of the computation remains the same. 
Thus, theoretically, our approach for the deterministic information  path can be expanded to the random information  path. 

Especially, the random information  path generalization can be directly solved by factoring in the path probability. However, this would require to compute the transition matrix for every ($u$,$v$) pair. 
This is much expensive than finding only the information  path.  
We will discuss this issue in next subsection. }


\comment{
it is not difficult to find both problems can be tackled by similar approach presented in the original problem. Especially, for the first problem, we basically needs to rewrite the saving of a path $r_{(u,v)}$ as $w(u,v)\times p(r_{(u,v)})$. 
This can be further factored into the savings of every connective backbone edges. 
What we need to do is instead of computing $N_1$ and $N_2$ using the number of information  path, but for each pair $u$ and $v$, computing the expected number of paths contain them, or contain such isolated occurrence.
The rest of the computation remains the same. 
Thus, theoretically, our approach for the deterministic information  path can be expanded to the random information  path. }

 

%\vspace*{-3.0ex}
\subsubsection{Research Issues to be Investigated}
%\vspace*{-2.0ex}
%We will investigate the following research issues for backbone extraction in the complex network: 

\noindent{\bf (A.1) Scalability:}}




%\subsubsection{Biological Applications of Information Backbone}

\comment{We plan to validate the backbone in two contexts. In the first context, we will use a transportation network, the Internet, or other network with a known backbone structure to see how many edges/nodes can be discovered by our backbone extraction problem. 
Second, we plan to extract and study network backbones from biological networks and social networks. In biological networks, we will try to understand the biological meaning of the backbone, by analyzing them under different biological conditions. 
In social networks, we plan to analyze how the backbone affects the communication structure. 
Also, we will study the {\em robustness} of backbones in terms of edge/vertex changes, and how sensitive they are with respect to parameters in the randomized information  path model. }

\comment{
\noindent{\bf (A.3) Backbone Robustness:}
How robust is the backbone? When the network changes such as edge/vertex removing or inserting, how much a backbone will change? 
Also, we are interested how sensitive it is with respect to parameters in the randomized information  path model. }


\comment{
\noindent{\bf (A.4) Relationship between Backbone and Modularity:}
How network backbone and modularity coexists and how they affect each? 
It seem the backbone emerge due to the long distance prefer information  path, while the modularity comes from the fact that a lot of communication takes in local places.
There have been little study on they  work together. 
We plan to analyze the backbone structure and the modularity structure on the biological network and social network and empirically study their relationship. }

\comment{
\noindent{\bf (A.3) Backbone Application:}
As discussed in the last section, one of my research focuses is on developing indices to answer distance queries or reachability queries on large graphs. 
A network backbone provides a tool for capturing the major traffic along the information  path connections. We plan to investigate how to apply the backbone structure to build indices for answering distance queries on large graphs. 
A particular angle we will explore is how to constrain the backbone to be a tree-shape and how this backbone-tree can be used in indexing.}



\comment{
3) Validation of backbones? 
How we can validate in real applications? 
A possible choice is in some applications, we have the backbone notation, can we use this method to detect it?
Secondly, we have to make a backbone, and then detect it from the real data? 
4) The interaction/relationship between modularity and backbone structure. }


%5) Application of backbones?
%How network backbone can be applied for database indexing and wireless network routing? 
%6) Further comparison of backbone and clustering, and its relationship? 



\comment{
There is advantage in more communication between hub nodes and non-hub nodes since it would allow a more concise organization structure. 


the the information  path on a tree can be simply de
(In man-made network, including traffic network and Internet, the backbone have higher bandwidth or faster communication cost. Those factors can be incorporated into the network as edge weight. But those in certain sense, can be looked at as the results of emergence of network backbone. If we are allow to reduce the energy cost, where we should invest to get better results. Even so, we still have the problem of how to recognize the backbone issue). 

For instance, if the 
This scheme can be generalized in considering the hierarchical notation of backbone (will be discussed later). 

 

 







In this project, we propose to apply a graph theoretical concept to model the network backbone. 

\noindent{\bf  (A.3.II) Random Walk, Clustering, and Backbone:} We also plan to investigate how the recently proposed ``randomized information  path''~\cite{CN:Yen08}, which generalizes the information  path and commute time (random walk) notation between two vertices, can be applied to capture the backbone notation. 
We also plan to study the relationship between clustering and backbone. For instance, we believe many of the backbone structures contain edges between different clusters. 
}

\comment{
\noindent{\bf (A.3.III) Variants:} This problem has many interesting variations. Especially, in the current formulation, we assume each pair of vertices has the same amount of communication requests,  What if we know }





\comment{
Also we plan to investigate how the recently proposed ``randomized information  path'' which generalize the information  path and random walk notation between two vertices can be applied to capture the backbone notation. 
We also plan to study the relationship between the clustering and backbone. For instance, we believe many of the backbone structures contains edges between different clusters. 
Finally, we plan to utilize the real transportation system, an email communication network and the metabolic network to validate our study. 
}


\comment{

\subsection{Clustering Typed Network}
In this work, we will study to effectively and efficiently cluster the typed network, where either each node has a type or each edge has a type, or both have a type.
In certain perspective, the typed network (graph) can be treated as a generalization of the directed graph, where an edge has only two types (in-link and out-link). 
Many applications, such as in social network analysis and biological network, the network can be formulated as typed network. 
To understand the structural properties of the network, not only the underlying topology, but also the type needs to be considered. 
However, little work has done to address clustering the typed network. 
The only related work we found so far in database/data mining community appears in this year's SIGMOD'08 ~\cite{}, where an OLAP type of analysis focused on utilizing the type information. 
In this project, we plan to study two problems of the clustering typed network. 

\subsubsection{Clustering with Type Information}
Here, we plan to directly apply the type information associated with the vertices and the edges for clustering purpose.
The intuition of the clustering typed network is to utilize the ``homogenous'' property: 
the vertices in the same clusters tends to share the same type. 
Similar properties can be applied to the edges: similar types of edges link the vertices of two clusters. 
Given this, we need to investigate how to incorporate such homogenous constraints into the clustering function. 
We believe the information theoretical criteria can be applied here. 
Simply speaking, we seek the best compression to transfer the graph with type information. 
If we do not consider the clustering, then, we need to transfer the type for each node 
and for the adjacency matrix, we need to transfer the type for each edge.
Thus, the cost of transferring the clustering result contains the cost of grouping assignment and their type information, denoted as \[N\times log(|C|)+\sum_{i=1}^{C} H(C_i)\], and the cost of edges in the clustering graph, ${|C| \choose 2} \times log |E| \times k$, where $C$ is the number of clusters, $|E|$ is the number of edges in the original graph, $H(C_i)$ is the entropy of the vertex type in the cluster $C_i$, and $k$ is the number of edge type in the network.  
Given the clustering graph, $L(G|C)$ will include the cost of transferring all the edges from one cluster to another and we can treat the no edge as an edge type as well: $\sum_{1\leq i,j\leq |C|}{L(C_{ij})|E_{ij}}$, where $L(C_{ij}|E_{ij})$ is the transfer cost for edge set from $C_i$ to $C_j$ given their edge type distribution is known. 
Thus, we can extend the information theoretical approach to cluster the typed graph. 
We are also interested in extending Newman's modularity for this setting. The main challenge here is how to define the ``null'' model. 
Recall in his original definition, the null model is considered the totally random graph model, i.e., the edges to connect vertices within a cluster and across the clusters are randomly distributed. 
Here, the ''null'' model has to consider the vertex type constraints and edge type constraints. 
We will investigate efficient techniques to identify the clustering for the typed network. 

\subsubsection{Discovering Motif-Constrained Community}
Network-motif is typically defined as ``frequent subgraph'' which appears frequently (or statistically significant) in the network. 
Much research has been done to discover network-motif in the network (typically, the network is labeled with type information). 
Furthermore, it has been shown that in many biological and man-made network, network motif is hown to be functional relevant, i.e., a network motif forms the basic functional units of the underlying system. 
However, little work has been done to study the relationship between the network motif and clustering. 
We believe by combining these two important techniques, we are able to get a better understanding the organizational and operational principles of the underlying system. 
In this project, we will study how to network motif can be used as a constraint for clustering. 
Our intuition is as follows: the clustering should not try to avoid the basic functional unit as less as possible. 
Alternatively, if we know certain basic units serves as the ``connection'' between different ``functional modules'', we will prefer to split the network using these basic functional unit. 
Thus, we formulate this problem as the constraint clustering problem, where the motif is served as the constraints. A user can specify how the motif should be treated in the clustering, for instance, either to avoid them or to split them, and even can specify based on the motif types. 

Even though constraint clustering has been studied for multi-dimensional clustering, little work has been done for the graph clustering. This is also the first study trying to address the algorithmic challenge on how to efficiently combine subgraph mining and clustering. 
A potential strategy to avoid the motif or to utilize the motif is to perform certain preprocessing: transform the ``motif'' into the edge weight. Then, then we can utilize the existing techniques to cluster the weighted network. 
However, the challenge is how to perform the transformation which can reflect our intuition on the cost of the split of the motif.
Another strategy to is to carry it out in an online fashion. 
Furthermore, since the motif discover is a rather costly process, an interesting research question is to integrate the motif discover process with clustering process. 



\comment{
There are other methods, such as utilizing edge-betweenness and clique perturbation. 
But majority of the clustering methods can be captured by these three categories. 
In this study, we will focus on these three categories. }
}

\comment{
3) the third category defines similarity/dissimilarity between pair of vertices and thus transforms the graph clustering problem back to the traditional data clustering problem~\cite{}. 
}




\comment{
Third, several investigation has been performed study the relationship between different similarity/dissimilarities for a pair of nodes and show the clustering method can employed by utilizing the kernel-tricks (based on the kernel-matrix based on the similarity measure). 
Then, utilizing the observation made by Dhillon {\em et. Al}, Kernel k-means is closely related to the graph cuts and spectral clustering, thus, we can compare these methods with the methods in the first category.} 

\comment{
\subsubsection{High-level structural matching (A.3.1)}
\vspace*{-2.0ex}

This tool search for the {\em clustering graph} of the complex network which best match a high-level structural description from the user. 
This tool can serve in a variety of applications: 
1) find the desired clustering based on the prior-knowledge of the user; 2) allow an interactive mining process, which allow user to guide and refine the clustering results; and 3)validating the uniqueness of the clustering results. 
Let $G=(V,E)$ the topology of the complex network.  
Let $G^q=(V^q,E^q)$ be the {\em query graph} (corresponding to the high level structural description of $G$), where $v_i \in V^q$ corresponds to a group of vertices in $V$ and $E_{ij}^q$ records user-desired edge density (or simply connectivity) between vertex $v_i$ and $v_j$ in $V^q$. 
Let $C[G]=(V^c,E^c)$ be the clustering graph derived from the clustering $C$, where each $v_i \in V_c$ corresponding to a cluster in $V$ and $E_{ij}^c$ records the edge density between cluster $i$ and $j$. 
For the matching purpose, we will assume both $E^q$ and $E^c$ represented in the {\em adjacency matrix} format, i.e., $E_{ij}^q$ and $E_{ij}^c$ are the elements in the $i$-th row and $j$-th column of their corresponding matrices. 

\bdefin{\bf (Structural Matching Problem)}
Given the complex network $G=(V,E)$ and query graph $G^q=(V^q,E^q)$, the structural matching problem searches for a clustering assignment $C: V\rightarrow V_q$, i.e. $C(v) \in V_q, v\in V$, such that the distance between the query graph adjacency matrix $E^q$ and the corresponding clustering graph adjacency matrix $E^c$ is minimized: 
\[\arg\min_{C} d(E^q,E^c) \]
Supposing the $L_p$ norm is used: $d(E^q-E^c||=(\sum_{i,j}||E_{ij}^q-E_{ij}^c||^p)^{1/p}$. 
Alternatively, we can apply the information theoretical criteria, such as the Kullback-Leibler divergence~\cite{}. 
\vspace*{1.0ex}
\edefin

\noindent{\bf (A.3.1.I) Efficient Matching Algorithm:}
The structural matching problem clearly generalizes the graph isomorphism (a special case when the query graph is as large as the original graph), which is still undecided between P and NP-hard.
Thus, finding the exact solution is very computationally expensive. 
We plan to investigate an efficient shuffling strategy to tackling this problem. 
The strategy will start from an initial random assignment, or from certain known clustering results. 
Then, it will continuously shuffle the vertices between the clusters to make the new clustering graph closer to the query graph. 
Specifically, instead of switching or changing the membership for one vertex pair or a single vertex at a time, our strategy is to perform $k$ such operation at one time. 
Alternatively, we may employ the shuffling strategy in Lin's algorithm~\cite{}. 
These strategies would allow us to employ the greedy strategy without falling into the local minimum easily. 
}

\comment{
In addition, we will also investigate an interesting variant of above problem: we allow user to specify the number of vertices for each cluster in the query graph and their total can be less than total number of vertices in $G$. Note that this problem turns out generalizes the subgraph isomorphism, which is an NP-hard problem. 
We will investigate how to apply our randomly shuffling strategy to this problem as well. 
}

\comment{
\noindent{\bf Subgraph Matching:} Recently, several work studies approximately subgraph matching~\cite{SAGA07,TALE08,CMU07}. However, our subgraph matching is at a much large scale. It matches the 
cluster graph with the query graph. }

\comment{
The second criteria for the dynamic module is an {\em information theoretical criterion}. 
The information theoretical approach has been successfully applied to bipartite graph~\cite{} and undirected graph~\cite{}. 
Here, we will expand it to our problem setting. 
In a nutshell, the information theoretical criteria aims to transfer the graph $G=(V,E)$ with the minimal description length (MDLP principle) by using the clustering results: 
$L(C[G])+L(G|C[G])$, 
where $L(C[G])$ is the message length for the {\em clustering graph} and $L(G|C[G])$ is the message length to transfer the original graph $G$ using $C[G]$. 
{\em Each vertex $i$ in $C[G]$ corresponds to a unique cluster $C_i$ in $G$, and each edge $E_{ij}$ in $C[G]$ records the the number of edges from cluster $C_i$ to $C_j$.} 

Given the clustering graph $C[G]$, the communication cost of transferring the original graph $G$ is the sum of the message length to transfer each edge sets between each cluster pair: 
$L(G|C[G])=\sum_{1\leq i,j\leq |C|}{L(C_{ij}|E_{ij})}$, where $|C|$ is the number of clusters, and $L(C_{ij}|E_{ij})$ is the cost of transferring the edge set from cluster $C_i$ to $C_j$. 
A good clustering would produce low entropy edge sets: some edge set very dense and some very sparse. 
However, this cost is balanced by the cost of transferring the clustering graph itself, which contains two components: the cost of cluster assignment, $N\times log(|C|)$, and the cost of transferring all the edge weights for the cluster graph, ${|C| \choose 2} \times log |E|$. 

However, this criteria does not necessarily produce densely connected clusters, i.e. $E_{ii}$ can be very sparse, or totally disconnected. 
To deal with this problem, we split the total communication cost $L(G)$ into two parts:
the first part $L_1$ is the cost of transferring all the edge sets within each cluster ($L_1=N\times log (|C|)+|C| \times log (|E|)+\sum_{i=1}^{|C|} L(C_{ii}|E_{ii})$) and the second part $L_2$ is for transferring the edge sets between clusters ($L_2=N\times log (|C|)+ \left({|C| \choose 2}-|C|\right) \times log (|E|)+ \sum_{1\leq i,j\leq |C|, i\neq j}{L(C_{ij}|E_{ij})})$.
\comment{  
\beqnarr
L_1&=&N\times log (|C|)+|C| \times log (|E|)+\sum_{i=1}^{|C|} L(C_{ii}|E_{ii}) \\
L_2&=&N\times log (|C|)+ \left({|C| \choose 2}-|C|\right) \times log (|E|)+ \sum_{1\leq i,j\leq |C|, i\neq j}{L(C_{ij}|E_{ij})} 
\eeqnarr }
Given this, our new information criterion for clustering is 
the linear combination of the both parts: 
$L(G)=\alpha L_1 + (1-\alpha) L_2, 0\leq \alpha \leq 1$. 
Note that when $\alpha=1/2$, we essentially have the typical transferring cost (reduce by a scale by 1/2). 
However, by adjusting $\alpha$, especially by reducing it close to $0$, we will be able to identify the more dense clusters. 
Interestingly, $L_1$ and $L_2$ have the direct correspondence to $G_1$ and $G_2$ for the generalized Newman's modularity. 
}
\comment{
In order to utilize these two criteria to perform clustering, we will investigate 
the following two important research issues: }



\comment{
In this project, we plan to investigate this problem from two perspectives:  
First, we plan to investigate the relationship of these methods. 
In particular, we would like to search for an unified framework where different methods can be expressed. 
Second, we plan to investigate how to evaluate and compare different methods, and this can help us identify their pros/cons.
\vspace*{-3.0ex}
\subsubsection{Graph Clustering Unification (A.2.1)}
\vspace*{-2.0ex}
}
\comment{
In this project, we plan to initially focus on two categories of graph clustering methods, which captures a majority of the existing clustering methods: 
1) the first category methods contains those recently proposed graph clustering algorithms, mainly from complex network research community.}


{\comment{
Different clustering approaches, including hierarchical methods~\cite{}, spectral analysis~\cite{}, and other optimization methods, such as simulated annealing~\cite{}, have been employed to cluster the graph by optimize the corresponding criteria.  



2) the second category of clustering methods are mainly developed by machine learning, pattern recognition, and data mining researchers. 
They typically employ the spectral methods to optimize the cut-based criteria~\cite{}, such as ratio association/ratio cut, normalized cut, MinMaxCut, etc. 
These criteria aim to minimize the number of edges between clusters (possibly with different normalization). 
}


\comment{
We also note that in general, the aforementioned causality test can be extended to nonlinear relationships. Existing studies have found that the linear Granger causality test (also corresponding to the vector autoregression) is a valid assumption for many real applications, such as gene expression and economics time series~\cite{granger,arnold07,CN:Fujita07,CN:OpgenRhein07}. }

\comment{
In this project, we will investigate how to formalize the notation of network backbone and how to extract it from massive complex networks efficiently. 

The key question we first need to address is that given a network topology, 
does it always exist a backbone? 
If there are backbones, how can formally define and capture it? 
}



\comment{
Our hypothesis here is that the network is organized in a way to speed up the information flow transfer in a cost effective way. Basically, even though the communication length between any two vertices does not need to be the shortest, however, the cost of the edges in the backbone tends to have lower cost and thus it becomes more cost effectively to communicate through the backbone. 
However, it is typically hard to know the cost of each edge in the complex network, and even this knowledge is given, it is not known how to model the backbone. }


\comment{
\subsection{Unification of Graph Clustering Methods} 
\vspace*{-2.0ex}
Over the last several years, several new graph clustering algorithms have been developed in the field of complex network analysis~\cite{Newman03,Newman04m,CN:Handcock07,CN:Hastings06,CN:Karrer08,CN:Rosvall08a}. 
These methods rely on a variety of criteria derived from statistics and information theory to capture the ``modularity'' notation. 
These criteria also seem quite different from the existing {\em cut-based} clustering criteria ~\cite{Shi00,Meila01,Zhou05,CN:Luxburg06}, such as ratio association/ratio cut, normalized cut, MinMaxCut.  These are typically solved by spectral methods, and have been extensively studied in the machine learning, pattern recognition and data mining fields over the last decade. 

However, we lack a systematic study of these existing algorithms.  
With so many clustering approaches, a fundamental question begs to be answered: (How) are these methods related to each other? 
Answering this question not only will lead to a better theoretically understanding of graph clustering, but also will provide us guidelines for applying these different methods. 

In this project, we start with the three best-known clustering criteria of recent years: Newman's modularity~\cite{Newman04m}, information theoretical criteria~\cite{CN:Rosvall08a}, and statistical inference criteria~\cite{CN:Hastings06}.
Our investigation is inspired by and builds upon our ICDM'07 data discretization unification paper~\cite{DBLP:conf/icdm/JinBM07} which shows that several seemingly different discretization methods -  utilizing Chi-square statistics, entropy criteria, statistical fitness measure, ({\em Akaike} information criterion (AIC), and Bayesian information criterion (BIC) - all share a common root from a statistical viewpoint.  
Even more surprisingly, we found all these methods can be unified based on a generalized entropy notation~\cite{DBLP:conf/icdm/JinBM07}. 

\noindent{\bf Unification of  Newman's Modularity,  Information Theoretical Criterion, and  Statistical Inference Criterion for Graph Clustering (A.2.I):}
Our preliminary investigation found a surprising link among those recently proposed modularity criteria, similar to the discretization study. First, Newman's modularity $Q$ is closely related to Cohen's Kappa coefficient~\cite{CN:Cohen60} (and also rediscovered as Newman's mixing coefficient~\cite{CN:Newman03Mixing}). 
This coefficient can be viewed as the squared and symmetric version of Pearson's chi-square $\chi^2$ statistics.
Second, $\chi^2$ statistics are asymptotically equivalent to $G^2$ statistics~\cite{CN:Agresti90}, which can be shown to be closely related to the Kullback-Leibler  divergence.
Note that both $\chi^2$ and $G^2$ statistics may serve as independence tests for a two-way contingency table. 
If we assume a multinomial distribution of a two-way contingency table, then the statistical fitness critieria (like AIC and BIC) can be applied for optimizing the parameters. 
However, it is not known how to compare these criteria analytically. In particular, how does the relationship between the two-way contingency table hold for the square contingency table? 
The square contingency table corresponds to the graph clustering scenario, where both columns and rows are the clusters in the graph. 
Further, how does Newman's modularity, which does not directly consider the degree of freedom and is unnormalized, capture the model complexity? Note that the MDLP and statistical fitness criteria explicitly consider such costs. 
Finally, is there a unified modularity function which can describe all these criteria? {\em This can even lead to a new and unified graph clustering approach.}
  
\noindent{\bf Unifying with Cut-based Spectral Criteria:}
There are several works which demonstrate the strong relationship between cut-based   spectral criteria different methods~\cite{CN:Luxburg06}.  
A recent work shows that Newman's modularity can be transformed to and solved by spectral methods as well~\cite{white05,Meila07}. 
This enables us to compare these different objective functions using the same format (all transformed to matrix trace-optimization problem). 
Particularly, we are interested in investigating how {\em random walk} can serve as the bridge to join the cut-based spectral criteria with these recent graph clustering criteria. 
Random walk has been extensively studied and analyzed in spectral analysis. However, it is unclear how the methods can be unified from a random walk viewpoint?
Interestingly, we note that a recent work shows a surprising relationship between random walk and the information theoretical criterion by considering the minimal length description for the random walk~\cite{CN:Rosvall08b}. 

\comment{
\noindent{\bf (A.2.III) Evaluation Criteria:}
Besides the analytically study of these different modularity and spectral criteria, we also hope to understand the pros/cons and limitations of these clustering methods under different clustering criteria. 
Specifically, we plan to compare the robustness~\cite{}, accuracy(precision/recall)~\cite{}, resolution~\cite{}, and scalability~\cite{} of these different clustering methods. 
We will develop a synthetic generator, which contains a variety of configurations, including allowing different cluster shapes, noise levels, and size adjustment, etc., for evaluating these methods in terms of these criteria. 
}


\subsubsection{Related Work}

As we mentioned before, many graph clustering algorithms~\cite{Newman03,Newman04m,CN:Handcock07,CN:Hastings06,CN:Karrer08,CN:Rosvall08a} have been recently proposed. However, little work has been done to understand the relationship of these different methods. 
Several researchers have shown the unification or the relationship between different spectral clustering methods and their ties to kernel $k$-means and nonnegative matrix factorization~\cite{Dhillon04,DBLP:conf/sdm/DingH05}. 
The unification of bi-clustering methods, which works on large bipartite graphs, has been performed from a matrix factorization perspective~\cite{DBLP:conf/kdd/Li05}. 

We have studied the unification of different discretization methods~\cite{DBLP:conf/icdm/JinBM07}. 
}

\comment{ 
The introducing of network backbone in the complex network can help minimize the path-recognition-path complexity. 
Considering there is a network backbone, the network traffic will very likely go through the backbone. 
For simplification, we can assume the communication is divided into three stages, from the starting vertex to the backbone, traveling in the backbone, and then, reaching the end vertex from the backbone. 
What makes backbone important is that it typically has a sparse structure and thus, enables much lower description cost of communication.
For instance, if the network backbone is a tree structure, then, the information  path can be much easier to describe. 
It is well-known constant-size node labeling enable shortest-path routing in trees where each node in the routing step only requires a constant-time decision. 
In general, if the subgraph is very sparse, each node will have a very small number of neighbors, we can design a coloring scheme so that for any node, each of its neighbors have a different color. Then we can assign each color a codeword. 
The number of total unique colors is bounded by the maximal degree of node in the sparse graph. 
Basically, the sparse graph simplifies the communication and enables each node to make a simpler routing decision. 

Figure~\ref{} shows the two level communication mechanisms involve the backbone. 
Basically, the network is partitioned in the two parts, the non-backbone part and backbone part, and each has a unique code associated with them. 
Figure~\ref{}(a) shows the original complex network. 
Figure~\ref{}(b) shows the code associated with each node and a represented information  path. 
Figure~\ref{}(c) shows the two level organization structure (including backbone structure and the coding associated with the backbone. 
Here, inside of the backbone, we are using the edge-labeling scheme to describe the path segments. [v1, v2, v3, b[e1, e2, e3]b, v4, v5] 
For illustration purpose, we use the Huffman codes here. 
Also, other type of coding can be used, but here we apply them to show the different coding costs for the non-backbone part and backbone part. 
The backbone's sparse structure need to be taken into consideration to reduce the code length. 
}


\comment{


 from a vertex $v$, and then random choose another vertex $v^\prime$; 
we walk from $v$ to $v^\prime$ through the information  path; 
then from $v^\prime$, we random select another target and reach it through the information  path.
In an infinite long walk, the visiting probability of each node will converge to $P(v)$. 
The entropy of the random walk is $\sum_{v} p_v \log p_v$, and its minimal description length is $N \times  \sum_{v} p_v \log p_v$. 

 
The most nature way for coding paths is to assign each node a unique codeword in the network and then each path is describe as the sequence of its nodes' codeword. 
Note that this code also corresponds to the most straightforward of routing scheme. 
Explicitly recording the information  path would allow the constant routing decision at each node on the information  path. 
Describe the path likely hood, and the reverse is its description length...}



\comment{
Given this, we can apply the recently proposed ``search information'' criteria which describe the information needed from a vertex to another vertex. 
The criteria is as follows: 
\[[P(p(s,t))]=\frac{1}{d(s)} \prod_{j \in p(s,t)} \frac{1}{k_s-1}\]
(This actually correspond to the edge coloring scheme. )
How to utilize the backbone? 
In backbone, we can select to enter the backbone and then in the backbone, we will make a choice. 
Thus, the navigation of using the backbone or not. 
There is a probability of entering and leaving the backbone. 
The probability of using the backbone can be defined as 
$(\frac{b_v}{d(v)})^{\beta_0}$ and exit probability $(\frac{b_v}{d(v)})^{\beta_1}$, where the parameter $\beta_0$ and $\beta_1$ shows an biased choice. 
In between, we will use the backbone to navigate. 

Based on the information theory~\cite{}, the recognition complexity of a path can be defined as the length of a code to describe it. 
The most nature way for coding paths is to assign each node a unique codeword in the network and then each path is describe as the sequence of its nodes' codeword. 
Note that this code also corresponds to the most straightforward of routing scheme. 
Explicitly recording the information  path would allow the constant routing decision at each node on the information  path. 
Describe the path likely hood, and the reverse is its description length...}


\comment{
As we will see, network backbone arises as the results of reducing the path recognition complexity without compromising energy cost.  
Let us consider the straightforward way of coding each individual node. 
This coding scheme is based on the probability of a node which appear in any information  path in the network. 
Let $P(v)$ be the fraction of information  paths through vertex $v$ among all the information  path.  
Without any prior knowledge, we can assume each pair of communication is equally likely. 
Thus, $P(v)$ commonly serve as the vertex centrality measure~\cite{}. 
Given this, assuming there is no high-level structures in the network (each node is independent in the information  path), to achieve the minimal length to describe all the information  paths, each node has the code length bounded by $log(P(v))$. 
This also corresponds to the following random walk on the complex network. 
We starts from a vertex $v$, and then random choose another vertex $v^\prime$; 
we walk from $v$ to $v^\prime$ through the information  path; 
then from $v^\prime$, we random select another target and reach it through the information  path.
In an infinite long walk, the visiting probability of each node will converge to $P(v)$. 
The entropy of the random walk is $\sum_{v} p_v \log p_v$, and its minimal description length is $N \times  \sum_{v} p_v \log p_v$. }

\comment{
Why network backbones emerge from the complex networks?  How to extract them systematically? What is the relationship between network backbone and network modularity? These open and fundamentally important questions in complex network mining which will be studied in the project. }
\comment{
By linking to the basic physical principles (energy efficiency), this framework demonstrate the surprising and also natural emergence of backbone structure in a complex network. 
This framework also describe an interesting link between the backbone structure and the widely studied modularity principle~\cite{}, and would allow to describe and mine both in a unified mathematical formulation.}

\comment{If there are several, we can have different options. 
We may make them equally likely, or choose the one with the minimal decoding cost. 
For the later case, if one uses the backbone, it is more likely to be chosen. 
Given this, we can define the overall coding cost for the information  path as: }

\comment{
All of the above relies on the explicitly use the coding of the expression. 
In the following, we propose a scheme which will simplify the description by using a simple path description principle. 
Thus, we introduce the following prune graph theoretical version of the backbone problem.  
Let $B=(V_B,E_B)$ be a connected subgraph of the complex network $G$. 
For any two vertices, $x$ and $y$, we define their communication through the backbone as follows. 
Let $x_b$ and $y_b$ be the closest vertices on the backbone which vertex $x$ and $y$ can reach, i.e., 
\[x_b=\arg\min_{z \in V_B} dis(x,z), \ \ \ y_b=\arg\min_{z \in V_B} dis(z,y) \]
Let $dis(x_b,y_b|B)$ be the shortest distance from $x_b$ to $y_b$ using only the vertices and edges in the backbone $B$. 
Given this, we define the distance between two vertices $x$ and $y$ using the backbone as $dis(x,B,y)=dis(x,x_b)+dis(x_b,y_b|B)+dis(y_b,y)$. 
Further, given an approximation ratio $\alpha$, for any two vertices $x$ and $y$, if their distance using the backbone, $dis(x,B,y)$ is within $1+\alpha$ times the information  path between them, $dis(x,y)$, we refer to this vertex pair as being {\em covered by the backbone}. 

\bdefin{\bf (Network Backbone Problem (Graph Theoretical))}
Given an approximation ratio $\alpha$, and two thresholds $\beta_V$ and $\beta_E$, the network backbone $B(V_B,E_B)$ is a connected subgraph, whose number of vertices and number of edges are less than $\beta_V|V|$ and $\beta_E|E|$, respectively, and which covers most vertex pairs:
\[\arg\max_{B} |\{(x,y),\frac{dis(x,B,y)}{dis(x,y)}\leq (1+\alpha)\}|,  \ \  \frac{|V_B|}{|V|}\leq \beta_V \ \ \& \ \  \frac{|E_B|}{|E|} \leq \beta_E \]  
\edefin

This formulation captures the intuition that the backbone facilitates the communication between the vertex pairs in the complex network. Note that different parameter values can suggest different backbones. 
We believe those different backbones can help to reveal the hierarchical organization of the backbone. 

Since there is no explicitly the coding cost, the first approach cannot be applied. 
However, the general idea can be applied here. 
The second strategy tries find a reasonably small core graph as the starting point for the removal. 
It involves two steps. 
In the first step, we plan to find $\beta_1$ vertices and $\beta_2$ edges independently which maximally cover the vertex pairs. (Here a vertex pair is covered by a vertex (edge), if its information  path go through the vertex (edge)). 
This step can be solved by a procedure similar to the $2$-HOP approach~\cite{Cohen:2002}. 
Given this, in the second step, we find the induced subgraph which contains all the vertices and edges discovered in the first step. Then, we will greedily remove edges and vertices to meet the threshold constraints. 
}

\comment{Instead, we propose a different approach to solve this problem.
The backbone discovery problem is likely to be an NP-hard problem, as it is related to the graph distance labeling problem~\cite{GPSPR04}. 
Our idea is to first build some basic components for the backbone. 
We will first identify the top length $k$ path who has the highest number of information  path go through them. 
This process can be achieved by a path argument process. We can combine the path 
Note that this process can be done in $O(N)$ time. 
Then, again, we will try to combine these paths so that their merged one can result in the most. 
In the process, we main a information  path index between any vertices in a connected components who are part of the backbone candidate. 
Then ...}


\comment{

If we replace an edge, we will reduce certain number of edges. 
However, adding the edge will increase the backbone cost...
Thus, we always choose the one with the maximal benefit and stop choosing until there is no increase...
Further, this may not be a connect subgraph, after that, we link this to be connected subgraph, 

In another variation, we consider biased information  path. 
This is based on the recently proposed notation. 
In the worst case, this becomes the totally random walk. 
Now our problem becomes clustering...
This demonstrate a deep relationship between clustering and backbone relations. 
}

\comment{
We can associate these two values with their corresponding edge-vertices and the edges in the second order graph. 
Given this, we associate each edge-vertex $v_e$ in the second order graph $G^\prime$, a weight $N_1(v_e)$ which records the number of isolated occurrence if this edge-vertex is in the backbone. For non-backbone edge-vertex, this weight is zero. 
We also associate each edge between two edge-vertices in $G^\prime$ with a weight recording the total number of information  paths which contains the consecutive edge-vertices, denoted as $N_2(v_{e1},v_{e2})$. 
Note that both weight can be computed rather efficiently. Especially, the latter one can be computed through a preprocessing since it is a constant for a given network. 
 


 
%$\delta_2(e_1,e_2)=C(e_1)+C(e_2)-(c_1+c_2+C_b(e_1)+C_b(e_2))>0$. 
% $\delta_1(e_b)=C(e_b)-(c_1+c_2+C_b(e_b))<0$, where $C(e_b)$ is the edge coding cost assuming it is not a backbone edge.
%However, if two connective edges of the backbone occur in a information  path together, it will have a saving: $\delta_2(e_1,e_2)=C(e_1)+C(e_2)-(c_1+c_2+C_b(e_1)+C_b(e_2))>0$. 
%Besides, we can only estimate the overall saving of a information  path by considering sum up the savings of every two connective backbone edges and the penalty of all isolated backbone edges in this path. 
%This forms a lower bound of the true coding saving, but enable a computationally efficient algorithmic solution for the backbone extraction problem. 
}

\comment{

After finding the weighted densest subgraph, we can quickly compute the weights $\delta_1$, $\delta_2$, and $N_1$. 
Then, we will be able to prune any edge-vertex is the removing of them can improve the overall coding saving. 
Finally, the pruned induced subgraph in the second order graph serve as our core to build the complete backbone.}

%The third step is performed in an incremental fashion. We can maintain 

 
\comment{
Our strategy to find the backbone is to first identify a core group of the edge-vertices in the backbone, which is likely to be beneficial to be included in the backbone. Then, we will perform the growing and shrinking process alternatively: we first start growing this partial backbone by adding edges into it. We grow it until there is no saving is possible by adding edge-vertices. 
Then, we will prune certain edges.
For the initial stage, we do not have the penalty for the isolated vertex, but we can have a reasonable penalty and saving for the edge vertices and the edges between them.
Thus, we would like to find an induced subgraph which as a high-saving cost. 
A possible choice can be a subgraph whose average saving is the highest. 
This problem corresponds to the densest weighted subgraph problem. The exact best solution is using the maximal flows problem, which has the bound. Another good approximation algorithm has $2$ approximation bound. 
For the growing step, we note that adding a vertex-edge to an existing backbone can 
induce two certain penalty and savings. Basically, the penalty increases and saving reduces. 
This process thus will results in less savings when the number of edge in the backbone expands. 
This problem can be expanded for a fixed number of edges, and select the best induced subgraph. 
[We need a figure to demonstrate these steps.] 
[Step 1: Densest subgraph, Step 2: Growing, Step 3: Shrinking]
A key question to work on is why adding an edge does not always good]. }



\comment{

Clearly, in most studies, those information does not provide to us. 

Taking those 
The ability to finding the backbone incorporating those 
 
In general, we may consider the optimal coding for each edge in a random walk context.  
Consider the following random walk, at each step, choosing another random vertex and take a information  path to reach it from the current vertex. 
Here, this random walk models a simple system communication behavior, i.e., each pair equally likely communicate. 
A more flexible assumption will be discussed later. 
%The entropy rate of this infinite random walk (edge sequence) will converge to  $-\sum_{(i,j) \in E} p(i,j)\times \log p(i,j)$ where $p(i,j)$ is the probability of a information  path takes edge $(i,j)$ when it go through  vertex $i$ (out of all the information  paths going through vertex $i$, the fraction of them directly connecting to vertex $j$). 
Under this model, the optimal coding cost of each edge $(i,j)$ in minimizing the description of this infinite random walk (edge sequence) is $\log \frac{1}{p(i,j)}$ ~\cite{}, 
where $p(i,j)$ is the probability of a information  path takes edge $(i,j)$ when it go through  vertex $i$ (out of all the information  paths going through vertex $i$, the fraction of them directly connecting to vertex $j$). 

Our first variants is to relax the constraints that one node has to use the information  path to reach another node. 
Rather, we utilize the recently proposed notation ``randomized information  path'', which generalizes treats both information  path and totally random walk between two nodes as a special case.

 
Given this, we will consider each edge and the consecutive ones using the probability notation. Our aforementioned method will still work. 
Most important, if the random walk is totally random, we can use this model to detect modularity structure. This is very closely related to the ~\cite{}, in which they use the node information compression to detect community. 
Here, we can apply a spectral clustering or recursive mincut to decompose the network. 
For instance, we can extract one community, and then drop all its surrounding edges. 
Then, we extract another one. Since we can expect the backbone will be in each local region... 
community structure is the backbone for the local random walk.

Those edge is very to be used by the local random walk. 
Or, we can simply apply the mincut split the network. It would produce an vertex-overlapped clusterings. (Very similar to what codense did). 
}

\comment{ 
Let us consider we just need information  path and suppose it is $(v_0,v_1,\cdots,v_k)$, where $u=v_0$ and $v_k=v$. 
Then, the transition  probability matrix $T$ has $T[v_{i-1},v_{i}]=1$ $1 \leq i \leq k$, where other cells are zero. 
If we consider only the random walk, then the transition probability matrix is defined by $T[u,v]=\frac{1}{d(u)}$ if $u$ and $v$ is adjacent. Otherwise $T[u,v]=0$. 
Basically, at each vertex, we randomly choose walking to its neighbor.}



\comment{
 
Assuming we have the transition probability matrix, each path from $u$ to $v$ will be associated with a probability by multiplying each transition probability. 
Besides, each path is associate with the path length or the walking distance from $u$ to $v$ by adding all the edge weight together along the path. 
Let $R$ be all the possible path from $u$ to $v$ including cycles. 
Then, we can derive the transition probably which can minimized the expected path length subject to a fixed relative entropy (Kullback-Leibler divergence) with respect to the natural random walk: 
\[\min{ \sum_{r\in R} p(r) D(r) } \mbox{ subject to } \sum_{r\in R}{p(r) \log \frac{p(r)}{p^n(r)}} =J_0\]
Here $J_0$ is a used specified priori. If it is $0$, we have the natural random walk, and when $J_0$ increases, the paths probability distribution is centered around the information  path. 
In ~\cite{}, an efficient linear algebra approach is developed to find the optimal transition probability to minimize the expected path length from $u$ to $v$ under the relative entropy constraints.

Now, in our problem, we assume every pair of vertices has such a priori, then, the problem is to find the backbone such that the overall expected coding length is minimized. {\em Given complex network $G$, the network backbone $B(V_B,E_B)$ is a connected subgraph, such that $\sum_{(u,v) \in V \times V} w(u,v) \times 
\sum_{r_{(u,v)} \in R_{(u,v)}} C(r_{(u,v)})p(r_{(u,v)})$ is minimal. }
}


\comment{
\noindent{\bf Graph Theoretical Generalization:}
In this generalization, instead of explicitly minimizing the path-recognition complexity, we consider a scheme which will simplify the path description by using the backbone. It seeks a tradeoff between the information  path and the sparse backbone structure. 
Let $B=(V_B,E_B)$ be a connected subgraph of the complex network $G$. 
For any two vertices, $x$ and $y$, we define their communication through the backbone as follows. 
Let $x_b$ and $y_b$ be the closest vertices on the backbone which vertex $x$ and $y$ can reach, i.e., 
\[x_b=\arg\min_{z \in V_B} dis(x,z), \ \ \ y_b=\arg\min_{z \in V_B} dis(z,y) \]
Let $dis(x_b,y_b|B)$ be the shortest distance from $x_b$ to $y_b$ using only the vertices and edges in the backbone $B$. 
Given this, we define the distance between two vertices $x$ and $y$ using the backbone as $dis(x,B,y)=dis(x,x_b)+dis(x_b,y_b|B)+dis(y_b,y)$. 
\comment{
Further, given an approximation ratio $\alpha$, for any two vertices $x$ and $y$, if their distance using the backbone, $dis(x,B,y)$ is within $1+\alpha$ times the information  path between them, $dis(x,y)$, we refer to this vertex pair as being {\em covered by the backbone}.} 
Our graph theoretical backbone problem is then formulated as follows: 
{\em 
Given an approximation ratio $\alpha$, and two thresholds $\beta_V$ and $\beta_E$, the network backbone $B(V_B,E_B)$ is a connected subgraph, whose number of vertices and number of edges are less than $\beta_V|V|$ and $\beta_E|E|$, respectively, and which covers most vertex pairs:
\[\arg\max_{B} |\{(x,y),\frac{dis(x,B,y)}{dis(x,y)}\leq (1+\alpha)\}|,  \ \ \frac{|V_B|}{|V|}\leq \beta_V \ \ \& \ \  \frac{|E_B|}{|E|} \leq \beta_E \]  }

This formulation shows the simplification of vertex-pair communication by 
maximizing the usage of backbone. However, this is in the cost of the longer path. 
Besides, we note that different parameter values can suggest different backbones and they can potentially help to reveal the hierarchical organization of the backbone. 
}

\comment{
Balancing of these two costs give arise to the network backbone structure: it captures the major usage of certain 

Network backbone gives arise 
However, the above coding does not utilize any correlation between consecutive moves occurring in the information  path. In many information  paths, certain edges tend to occur consecutively. For example, in Figure~\ref{}, edge $e_1, e_2$ appear together in many information  paths.
In this case, if we extract their common prefix,  for instance, we may reduce the description of those information  path who include both consecutively. 
Besides, we also know a sparser graph is easier to navigate and tends to have lower coding cost. 
These two observations form the basis for the emergence of backbone: a sparse subgraph where many consecutive edges in the information  paths are linked together.}



==> Directed.tex <==
\section{Algorithm for Directed Graph}
\label{directed}

Our approach will distribute the global optimization problem into the subproblem of each vertex, and then extract the backbone from the viewpoint of graph theory.
Specially, in the first step, we optimize the subproblem of each vertex in order to extract the candidates of backbone edges,
and generate a vertex-weight graph, so-called backbone graph, to describe the topological relationships among them.
In the second step, we formulate the backbone discovery problem of network as the ``maximum-weight connected graph'' problem in backbone graph,
and solve it using existing heuristics.
Next, we discuss these two steps in details.


\subsection{Backbone Edge Discovery on Incoming Edges}
\label{bediscovery}

%Given the probability distribution table for each vertex (as illustrated in Figure \ref{bicl}), following equation is a
%constant:
%\[ C(v) = \prod_{e_i \in in(v), e_j \in out(v)} p^{N_{ij}} (e_j | e_i) \]
%We apply $log$ conversion on $C(v)$ and obtain
%\[ \log C(v) = \sum_{e_i \in in(v), e_j \in out(v)} N_{ij} \log p(e_j|e_i) \]

Recall that our goal aims to reduce the number of parameters while preserving good modeling accuracy which is comparable with likelihood model in Eq. \ref{condprob}.
Clearly, significant reduction of the number of parameters can be achieved utilizing backbone (as likelihood function $\mathcal{L}(p)$ in Eq. \ref{bbmdl}).
Thus, the remaining issue is to maximize the ratio between likelihood function in Eq. \ref{condprob} and Eq. \ref{bbmdl}, i.e.,
{\tiny
\beqnarr
\frac{\prod_{e_i \in E} p^{N_i^\prime}(e_i) \prod_{v \in V} [\prod_{e_i\in out(v)} p^{N^B_i}(e_i | B_v) \prod_{e_j\in out(v)} p^{N^{\bar{B}}_j}(e_j | \bar{B_v})]}{\prod_{e_i \in E} p^{N_i^\prime}(e_i) \prod_{e_i, e_j \in E} p^{N_{ij}}(e_j|e_i)} \nonumber \\
= \frac{\prod_{v \in V} [\prod_{e_i\in out(v)} p^{N^B_i}(e_i | B_v) \prod_{e_j\in out(v)} p^{N^{\bar{B}}_j}(e_j | \bar{B_v})]}{ \prod_{e_i, e_j \in E} p^{N_{ij}}(e_j|e_i)}
\eeqnarr
}
Note that, given the probability distribution table for each vertex (as illustrated in Figure \ref{bicl}), the denominator is a constant.
For each vertex, it is equivalent to maximizing
\beqnarr
\label{subobj}
\sum_{e_i\in out(v)} N^B_i \log p(e_i | B_v) + \sum_{e_j\in out(v)} N^{\bar{B}}_j \log p(e_j | \bar{B}_v)
\eeqnarr
Combining the aforementioned constant with sub-objective function, we have
{ \small
\beqnarr
\label{funcF}
F = \sum_{e_i \in in(v), e_j \in out(v)} N_{ij} \log p(e_j|e_i)  \nonumber \\
    - \sum_{e_j \in out(v)} ( N^B_j \log p(e_j | B_v) + N^{\bar{B}}_j \log p(e_j | \bar{B}_v)) \\
  = (\sum_{e_i \in B_v} \sum_{e_j \in out(v)} N_{ij} \log p(e_j|e_i) - \sum_{e_j \in out(v)} N^B_j \log p(e_j | B_v)) \nonumber \\
  + (\sum_{e_i \in \bar{B}_v} \sum_{e_j \in out(v)} N_{ij} \log p(e_j|e_i) - \sum_{e_j \in out(v)} N^{\bar{B}}_j \log p(e_j | \bar{B}_v) ) \\
  = \sum_{e_j \in out(v)} [ (\sum_{e_i \in B_v} N_{ij} \log p(e_j|e_i) - \sum_{e_i \in B_v} N_{ij} \log p(e_j | B_v)) \nonumber \\
  +(\sum_{e_i \in \bar{B}_v} N_{ij} \log p(e_j|e_i) - \sum_{e_i \in \bar{B}_v} N_{ij} \log p(e_j|\bar{B}_v) ) ] \\
  =  \sum_{e_j \in out(v)} [\sum_{e_i \in B_v} N_{ij} \log \frac{p(e_j|e_i)}{p(e_j|B_v)} + \sum_{e_i \in \bar{B}_v} N_{ij} \log \frac{p(e_j|e_i)}{p(e_j|\bar{B}_v)}]
\eeqnarr
}
where $p(e_j | B_v) = \frac{N^B_j}{\sum_j N^B_j}$ and $p(e_j | \bar{B}_v) = \frac{N^{\bar{B}}_j}{\sum_j
N^{\bar{B}}_j}$, if  $p(e_j | e_i) = \frac{N_{ij}}{\sum_j N_{ij}}$ is given. As we see, optimization of sub-objective
function is the same with minimizing function $F$. Here, we can interpret $p(e_j|B_v)$ and $p(e_j|\bar{B}_v)$ are
``centers'' for two clusters. And thus, the function $F$ serves as the objective of minimizing the within-cluster
distance, which actually is the goal of k-means style algorithm. The different thing is that we apply new distance metric
based on K-L divergence instead of Euclidean distance in traditional k-means algorithm. Follow the procedure of
k-means, the backbone edges from each vertex' incoming edges are extracted. Furthermore, we assign a weight to each
vertex as the value of sub-objective function in Eq. \ref{subobj}.
The outline of algorithm is introduced in Algorithm \ref{alg:kmeans}.

\input{Figures/KMeans.tex}


\subsection{Maximum Weight Connected Graph}
\label{mcg}

In the following, we transform the backbone discovery problem of maximizing likelihood function in Eq. \ref{bbmdl} into
a maximum weight connected graph problem (MCG). The intuition is that if the sum of weights of a set of connected
vertices is maximal, the optimality of Eq. \ref{bbmdl} is also achieved and corresponding subgraph connected by
extracted backbone edges is found.

Given this, we introduce a {\bf backbone graph} aggregating all extracted backbone edges. Specially, {\bf backbone
graph} $G^B = (V,E^B)$is a vertex-weight directed graph, where $V$ is the vertex set in the network $G$, and an edge
$(v_i, v_j)$ exists if this edge is extracted backbone edge with respect to vertex $v_j$. If we can find a set of
connected vertices which maximize the sum of their vertex weight in $G^B$, its corresponding induced graph clearly
optimizes likelihood function $\mathcal{L}(p)$, since it is the product of all probability items related to included
vertices.
Moreover, given a positive integer $k$,
the problem of maximum weight connected graph (MCG) is to identify a connected subgraph with $k$ vertices which maximize the sum of their weight in vertex-weight graph.
The most variant of maximum weight connected graph (MCG) is constrained maximum weight connected graph (CMCG) where a predetermined vertex is required to be contained in the resulting graph.
These problems have various application on communication network design.
Thus, we can see the backbone discovery problem is an instance of maximum weight connected graph (MCG) problem.
The maximum weight connected graph (MCG) problem is well-studied problem in the field of graph theory, which has been proved to be NP-hard.
We can apply the heuristic algorithm introduced in \cite{Lee98} here.
The basic idea is to decompose MCG into several small CMCGs and invoke the subroutine for CMCGs which is also proposed by Lee and Dooly \cite{Lee96}.
Specially, all vertices are first ranked by certain criteria.
Following this order, each vertex is added into the graph and is determined to be the vertex which should be included.
Then, we call the subroutine for CMCG to solve it.
This procedure is repeated for all vertex and the subgraph with maximal sum of vertices weight is taken as the final result.
The sketch of heuristic algorithm for MCG is provided in Algorithm \ref{alg:mcg}.
Interested readers please refer to \cite{Lee98} for details.

\input{Figures/MCG.tex}


\subsection{Overall algorithm and complexity analysis}

The overall procedure to discover backbone in directed graph involving three steps.

\noindent \textbf{step 1:} we preprocess the network to enumerate all shortest paths for computing edge betweenness and segment betweenness
(i.e., the number of shortest paths passing through these consecutive edges. The length of segment is 2 in this work).
Then, the probability distribution table for each vertex is constructed for further backbone edge extraction.

\noindent \textbf{step 2:} given probability distribution table, we extract backbone edges from each vertex' incoming edges.
Follow that, the vertex-weight directed graph, so-called \textbf{backbone graph}, is generated,
where each vertex is assigned the weight as the value of Eq. \ref{subobj}.

\noindent \textbf{step 3:}
we transform the problem of discovering backbone into ``maximum weight connected graph'' problem and solve it by existing heuristics.

The complexity of our approach is as follows.
In the first step, we have to compute all pairs of shortest distance and utilize the following observation to compute edge or segment betweenness
\[dist(u,v) = dist(u,x) + dist(y,v) + length(x,y)\]
That means if shortest path from $u$ to $v$ passing through segment $x\rightarrow y$, then above equation is satisfied, and vice versa.
We can invoke $|V|$ times BFS procedure in $O(|V|\times(|V|+|E|)$.
Then, it takes at most $O(|V| TC(G))$ to compute the edge betweenness or segment betweenness, where $TC(G)$ is the size of transitive closure of network $G$.
Therefore, step 1 costs $O(|V| TC(G))$ in worst case.
In step 2, it takes $O(|out(v)|)$ time for each iteration.
Assuming the number of iteration is $K^\prime$, for each vertex, the biclustering algorithm takes $O(K^\prime \times |out(v)|)$.
Thus, the step 2 needs $O(K \times |E|)$ time if $K = max(K^\prime)$ for all vertices.
For the last step, if we apply heuristic algorithm $DEP\_HEU$ to solve CMCG in $O(k^2|V|+k|E|)$ time (introduced in \cite{Lee96}),
it totally takes $O(k^2|V|^2+k|V||E|)$ time to find maximum weight connected graph, where $k$ is the number of vertices in resulting graph.
Overall, the time complexity of backbone discovery algorithm in directed graph is $O(|V| TC(G) + K |E| + k^2 |V|^2 + k|V| |E|)$.
It is not hard to see the first step of constructing probability distribution table dominates the computational cost of this algorithm.


==> Figures/Bicluster.tex <==
\begin{algorithm}[t!]
\caption{Biclustering($D,D^T$)}
\label{alg:biclustering}
\begin{algorithmic}[1]
\STATE randomly choose initial centroid $c_1$ and $c_2$ for both $D$ and $D^T$;
\REPEAT
    \STATE assign each edge $e_i$ to the cluster with the closest distance in $D$ and $D_T$, such that Eq. \ref{dist} is satisfied;
    \STATE update centroids of clusters in $D$ and $D^T$, individually;
\UNTIL{stop criteria is satisfied}
\end{algorithmic}
\end{algorithm}


==> Figures/CoreGen.tex <==
\begin{algorithm}
\caption{Pruning($G^\prime$,$k_0$,$k_1$)}
\label{alg:prune}
\begin{algorithmic}[1]
\REQUIRE $k_0$ is the number of edges in each sampled subgraph and $k_1$ is the number of edges in resulting core;
\STATE $G_c \leftarrow G^\prime$;
\WHILE{$|V(G_c)| > k_1$}
    \STATE $G_s \leftarrow G_c$;
    \STATE $G_c \leftarrow \emptyset$;
    \REPEAT
        \STATE call GreedyAlgorithm$(G_s,k_0)$ or LocalSearch$(G_s,k_0)$ to obtain a sampled subgraph $G_0$;
        \STATE update $N_1$ for each vertex in $G_0$ assuming $G_0$ is the backbone;
        \STATE estimate $\delta_1$ and $\delta_2$ for each vertex and edge in $G_0$;
        \STATE calculate the value of objective function $c$ given new $N_1$ and $N_2$;
        \STATE randomly remove one edge included in $G_0$ from $G_s$;
        \STATE $G_c \leftarrow G_a \cup G_0$;
    \UNTIL{$c$ is not significantly changed};
\ENDWHILE
\RETURN $G_c$;
\end{algorithmic}
\end{algorithm} 

==> Figures/DFSExp.tex <==
\begin{algorithm}
\caption{Expand($G$,$G_0$,$r$)}
\label{alg:expand}
\begin{algorithmic}[1]
\IF{$r \le 0$}
    \RETURN $G_0$;
\ENDIF
\STATE add the vertex $u \in (G \setminus G_0)$ incident to $G_0$ and has maximal weight to $G_0$;
\STATE $r \leftarrow r - 1$;
\STATE recursively invoke $Expand(G,G_0,r)$ to incrementally generate $G_0$;
\end{algorithmic}
\end{algorithm}


==> Figures/Enum.tex <==
\begin{algorithm}[t!]
\caption{BackboneSearch($G^\prime, k, P, N, Ex$)}
\label{alg:enumeration}
\begin{algorithmic}[1]
\REQUIRE $k$ \{the number of edges in original graph\}
\REQUIRE $P$ \{the set of edge-vertices in $G^\prime$ currently in the connected subgraph\}
\REQUIRE $N$ \{the set of edge-vertices in $G^\prime$ that can be added into the current subgraph\}
\REQUIRE $Ex$ \{the set of edge-vertices in $G^\prime$ that have been previously expanded\}
\IF{$P \setminus Ex = \emptyset$ and $|P| = k$}
    \STATE compute the value of objective function $cost(P)$;
    \IF{$cost(P) > max\_cost$}
        \STATE $max\_cost \leftarrow cost(P)$;
        \STATE $B \leftarrow G_s(P)$; \COMMENT{$G_s(P)$ is the subgraph induced by the edge set $P$ in original graph}
    \ENDIF
\ELSE
    \IF{$|P|<k$}
        \FORALL{edge-vertex $e \in N$}
            \STATE BackboneSearch($G^\prime,k, P\cup\{e\}, N \cap Nei(e), Ex \cap Nei(e)$); \COMMENT{$Nei(e)$ is the neighboring set of $e$ in $G^\prime$}
            \STATE $N \leftarrow N \setminus \{e\}$;
            \STATE $Ex \leftarrow Ex \cup \{e\}$;
        \ENDFOR
    \ENDIF
\ENDIF
\end{algorithmic}
\end{algorithm} 

==> Figures/Gen2Means.tex <==
\begin{algorithm}
\caption{Generalized2Means($G_0$)}
\label{alg:gen2means}
\begin{algorithmic}[1]
\REPEAT
    \FORALL{edge $e=(v_s,v_t) \in E(G_0)$}
        \STATE assign the edge $e$ as non-backbone edge if inequality \ref{dist} is satisfied;
        \IF{$e$ is non-backbone edge}
            \STATE update the centroids of probability distribution tables $D_s$ and $D_t$;
            \STATE update the value of objective function on probability distribution tables $D_s$ and $D_t$;
        \ENDIF
    \ENDFOR
\UNTIL{no edge's cluster membership is changed}
\RETURN sum of updated vertex weights
\end{algorithmic}
\end{algorithm}


==> Figures/Gen2Means_bak.tex <==
\begin{algorithm}
\caption{Generalized2Means($G_0$)}
\label{alg:gen2means}
\begin{algorithmic}[1]
\FORALL{edge $e=(v_s,v_t) \in E(G_0)$}
    \REPEAT
        \STATE assign the edge $e$ to the cluster with smallest sum of distance such that inequality \ref{dist} is satisfied;
        \STATE update the centroids of probability distribution tables $D_s$ and $D_t$, individually;
        \STATE update the value of objective function on probability distribution tables $D_s$ and $D_t$;
    \UNTIL{$e$'s cluster membership is stable}
\ENDFOR
\RETURN sum of updated vertex weights;
\end{algorithmic}
\end{algorithm}


==> Figures/Greedy.tex <==
\begin{algorithm}
\caption{GreedyAlgorithm($G^\prime$,$k$)}
\label{alg:greedy}
\begin{algorithmic}[1]
\FORALL{edge $(e_1,e_2) \in E(G^\prime)$}
    \STATE score $s(e_1,e_2) \leftarrow \delta_2(e_1,e_2) \times N_2(e_1,e_2)+\delta_1(e_1)\times N_1(e_1)+ \delta_1(e_2) \times N_1(e_2)$;
\ENDFOR
\WHILE{some edge scores are positive \textbf{and} $|E(G_H)|<k$}
    \STATE insert the edge with largest score into heaviest subgraph $G_H$;
    \IF{endpoint $e_1$ or $e_2$ is included in $G_H$ at first time}
        \STATE the scores of edges incident to $e_1$ or $e_2$ are updated by $\delta_1(e_1) \times N_1(e_1)$ or $\delta_1(e_2)\times N_1(e_2)$, respectively;
    \ENDIF
\ENDWHILE
\RETURN $G_H$;
\end{algorithmic}
\end{algorithm} 

==> Figures/IterDis_bak.tex <==
\begin{algorithm}
\caption{DiscoveryBackbone($G=(V,E)$,$K$)}
\label{alg:iterativealg}
{\small
\begin{algorithmic}[1]
\REQUIRE{ $G$ is the input graph, $K$ is the backbone size} \\
\COMMENT{Step 1: Preprocessing}
\FORALL {$u \in V$}
     \STATE invoke {\em Bi-KL-Partition}(u);
     \STATE compute $F(u)$;
\ENDFOR \\
\COMMENT{Step 2: Starting Candidate Backbone}
\STATE $V_s \leftarrow MCG(V,K)$;
\STATE $W_H \leftarrow \sum_{u \in V_s} F(u)$;
\STATE $\mathcal{B} \leftarrow$ {\em GBi-KL-Partition($V_s$)};
\STATE $W_L \leftarrow \sum_{u \in V_s} F^\prime(u)$; \COMMENT{$F^\prime(u)$ is under the updated parameters of $p(e|\mathcal{B})$ and $p(e\overline{\mathcal{B}})$}
\STATE $W \leftarrow W_L$; \\
\COMMENT{Step 3: Iterative Improvement}
\WHILE{$|V(G)| > K \wedge W_H > W$}
    \STATE randomly remove one vertex $v$ from $G$;
    \STATE $V_s \leftarrow V_s \backslash \{v\}$;
    \STATE $u \leftarrow \arg\max_{u \in \mathcal{N}(V_s)} F(u)$;
    \STATE $W_H \leftarrow  W_H-F(v)+ F(u)$;
    \STATE $\mathcal{B} \leftarrow$ {\em GBi-KL-Partition($V_s$)};
    \STATE $W_L=\sum_{u \in V_s} F^\prime(u)$;
    \IF{$W < W_L$}
        \STATE $W \leftarrow W_L$;
        \STATE $G_B \leftarrow (V_s,\mathcal{B})$; \COMMENT{keep the best result}
    \ENDIF
\ENDWHILE
\RETURN $G_B$;
\end{algorithmic}
}
\end{algorithm}


==> Figures/LocalSearch.tex <==
\begin{algorithm}
\caption{LocalSearch($G^\prime$,$k$)}
\label{alg:localsearch}
\begin{algorithmic}[1]
\FORALL{vertex $e_i \in V(G^\prime)$}
    \STATE score $s(e_i) \leftarrow \sum_{e_j \in Neighbor(e_i)} (\delta_2(e_i,e_j) N_2(e_i, e_j) + \delta_1(e_i) N_1(e_i))$;
\ENDFOR
\STATE start from the vertex with largest score and apply BFS to collect $k$ vertices (the vertices with larger scores have higher priority to be visited);
\STATE extract initial subgraph $G_H$ induced by collected $k$ vertices;
\REPEAT
    \STATE evaluate the improvement of each possible swap between the vertices inside and outside the subgraph which are connected by the edges;
    \STATE apply the swap with largest improvement and update the subgraph $G_H$;
\UNTIL{no improvement by swaping can be achieved}
\RETURN $G_H$;
\end{algorithmic}
\end{algorithm} 

==> Figures/MCG.tex <==
\begin{algorithm}[t!]
\caption{MCG($G$, $k$)}
\label{alg:mcg}
\begin{algorithmic}[1]
\STATE rank all vertices $V(G)$ by certain criteria;
\STATE $G_{k-1}$ is initialized as the induced subgraph with first $k-1$ vertices;
\STATE $w(G_{k-1})$ is the sum of vertices weight in $G_{k-1}$;
\FOR{$i = k$ to $|V|$ (follow the order of vertices)}
    \STATE add vertex $v_i$ to $G_{i-1}$;
    \IF{$V(G_i) \ge k$}
        \STATE call subroutine for CMCG with fixing vertex $v_i$;
        \IF{$max\_weight \le w(G_i)$}
            \STATE $max\_weight \leftarrow w(G_i)$;
            \STATE set $G_i$ as the maximum connected subgraph;
        \ENDIF
    \ENDIF
\ENDFOR
\end{algorithmic}
\end{algorithm}


==> Figures/RealData.tex <==
\begin{table}
\begin{center}
{\small
\begin{tabular}{|l|c|c|r|}
\hline Dataset &  \#V  & \#E   & Density \\ \hline
AgroCyc & 13969 & 17694 & 1.27 \\ \hline
Ecoo157 & 13800 & 17308 &
1.25 \\ \hline GO      & 6793  & 13361 & 1.97 \\ \hline HpyCyc  & 5565  & 8474  & 1.52 \\ \hline Nasa    & 5704  & 7942
& 1.39 \\ \hline P2PG08 & 4055 & 12443 & 3.07 \\ \hline P2PG09 & 4179 & 11944 & 2.86 \\ \hline Reactome& 3678  & 14447
& 3.93 \\ \hline Vchocyc & 10694 & 14207 & 1.33 \\ \hline Xmark   & 6483  & 7654  & 1.18 \\ \hline
\end{tabular}
}
\end{center}
%\vspace{-2.0ex} 
\caption{Real datasets} \label{realdata}
\end{table}


==> Figures/Trafficnet.tex <==
\begin{figure*}[tbp]

\resizebox{\textwidth}{!} {
\begin{minipage}[c]{0.75\textwidth}
\centering

    \mbox{
        \subfigure[Network and its backbone]{\includegraphics[width=1.5in,height=1.2in]{Figures/backbone.eps}\label{f1}}
    }
    \mbox{
        \subfigure[Coding of subgraph]{\includegraphics[width=1.5in,height=1.2in]{Figures/graphcoding1.eps}\label{f2}}
    }
    \mbox{
        \subfigure[Path coding example]{\includegraphics[width=1.5in,height=1.2in]{Figures/pathcoding.eps}\label{f3}}
    }


\caption{Path encoding with and without backbone}
\label{fig:graphcode}
\end{minipage}
\hspace{0.02cm}


\begin{minipage}[c]{0.25\textwidth}
\centering
\psfig{figure=Figures/trafficnetwork.eps,scale=0.55}

\caption{ Traffic Network }
\label{fig:trafficnetwork}
\end{minipage}
\hspace{0.02cm}
}
\end{figure*}


==> IterativeAlg.tex <==
\section{Iterative Graph Reduction Algorithm}
\label{iterative}

In this second, we propose a new scheme by iteratively invoking the approach for heaviest k-subgraph problem to discover network backbone.
During the procedure, two parameters penalty $\delta_1$ and $\delta_2$ are also estimated.
Specially, network backbone is extracted in two steps. First, the core of backbone is generated by a pruning procedure which consists of sampling and assembling steps. Then, since the backbone core is small enough, we apply enumeration technique to find a optimal backbone in a brute force manner.

\subsection{Pruning}
\label{pruning}

We first introduce the graph pruning scheme for extracting the core of backbone. Here, we consider backbone ``core'' as the superset of backbone, i.e., backbone is included in the ``core''.
Recall our problem is to find a subgraph which has $k$ edges and maximizes $ \sum_{e \in V^\prime(B)} N_1(e) \times \delta_1(e) + \sum_{(e_1,e_2) \in E^\prime(B)} N_2(e_1,e_2) \times \delta_2(e_1,e_2)$.
This is problem is quite challenging because all four values $N_1$, $N_2$, $\delta_1$ and $\delta_2$ are unknown if backbone is not discovered.

To solve the problem, we first gain a better understanding of objective function. From the viewpoint of graph, if we take the original network as backbone, i.e., $N_1$ is set to 0, the value of objective function is overestimated.
The basic idea of our scheme is that, starting from this overestimated initial graph, we iteratively decrease it by pruning some edges in the graph.
Specially, the pruning is achieved by sampling one network several times and assemble those samples to generate the resulting graph.
That it, the edges which are not included in the resulting graph is said to be pruned.
This resulting graph is taken as the input the graph pruning in next iteration.
We will repeat this pruning procedure several times until resulting graph is small enough which serve as the ``core'' of backbone.
The entire pruning scheme is outlined in Algorithm \ref{alg:prune}.

\input{Figures/CoreGen.tex}

Moreover, the parameter of penalty $\delta_1$ and saving $\delta_2$ are also estimated during the pruning process.
Given the backbone, with each vertex $e$, $\delta_1(e)$ is represented as the relative improvement of local coding length on $e$ with backbone compared with the one without backbone.
Considering a relatively extreme case, someone would note that if one edge is included by a small number of shortest paths, the coding length of this edge should be very long.
And if this edge is contained in the backbone, the coding length of this edge in the backbone would be significantly reduced even some extra costs (e.g., entering and exiting codes) are added.
In this case, $\delta_1$ is positive and also should be viewed as saving.
However, we can see that $N_1(e)$ and $\delta_1(e)$ are combined together in the objective function and $N_1(e)$ is very small in this case.
Therefore, from a globe viewpoint, this type of small saving is not encouraged in our objective function which can be taken as a variant of penalty.
Likewise, for each edge $(e_1,e_2)$, $\delta_2(e_1,e_2)$ is expressed as the relative improvement of local coding length on $(e_1,e_2)$ with backbone compared with the one without backbone.
Assuming we only re-encode the edges within backbone while keeping the original codes for non-backbone edges, the penalty and saving can be formally expressed as
\[\delta_1(e) = l_G(e) - (l_B(e)+B_{in}+B_{out}) \]
\[\delta_2(e_1,e_2) = l_G(e_1,e_2) - (l_B(e_1,e_2)+B_{in}+B_{out})\]
where $l_G(e)$ and $l_G(e_1,e_2)$ are coding length of edge $e$ and segment $(e_1,e_2)$ in original graph, and $l_B(e)$ and $l_G(e_1,e_2)$ are coding length of edge $e$ and segment $(e_1,e_2)$ in the backbone.
Note that, $B_{in}$ and $B_{out}$ are the coding length of two special symbols to indicate entering and exiting of backbone.

Since we have to generate distinguishable codes to indicate the entrance and exit of backbone, the coding length of those entering and exiting indicators are important for computing $\delta_1$ and $\delta_2$.
Intuitively, shorter the entering and exiting codes are, more saving on coding cost can back obtain.
A naive solution is to define a coding rule such that the first bit of each edge codes is used to indicate whether this edge is included in the backbone or not.
Clearly, the overall cost is significantly increased.

\begin{figure*}[t!]
    \centering
    \mbox{
        \subfigure[Entrance coding]{\includegraphics[width=2in,height=1.5in]{Figures/entrance.eps}\label{entrance}}
    }
    \mbox{
        \subfigure[Exit coding]{\includegraphics[width=2in,height=1.5in]{Figures/exit.eps}\label{exit}}
    }
    \caption{Local coding of entrance and exit symbols}
    \label{fig:symbols}
\end{figure*}


\subsection{Coding Scheme}
\label{coding}

In the following, we investigate the relationship between the coding scheme and saving cost to propose a local coding approach for entering and exiting symbols.
Essentially, the cost saving for coding length is achieved by encoding the backbone edges and non-backbone edges from the perspective of each vertex.
That is, assuming coding of non-backbone edges are not changed, the coding length of backbone edges are significantly reduced.
As discussed, we have to assign two special codings for entrance symbol ``['' and exit symbol ``]''.
Specially, with regard to entrance symbol ``['' (as shown in Figure \ref{entrance}), the outgoing edges is decomposed into two categories: non-backbone edges and backbone edges.
In figure \ref{entrance}, we use one virtual vertex to indicate the starting point of backbone edges.
The coding of exit symbol ``]'' is similarly illustrated in Figure \ref{exit}.
From the viewpoint of vertex which has both incoming and outgoing edges, there are four events possibly occurred with regard to previous and next edges: case 1) from non-backbone edge to backbone edge by indicating ``[''; case 2) from non-backbone edge to non-backbone edge; case 3) from backbone edge to non-backbone edge by indicating ``]''; and case 4) from backbone edge to backbone edge (keeping the coding inside ``[]'').
Taking the coding cost saving into consideration, we encode the combination of entrance symbol ``['' and non-backbone edges (case 1 and case 2), and the combination of exit symbol ``]'' and backbone edges (case 3 and case 4), separately.
We refer the coding book for case 1 and 2 as $Inbook$, and the coding book for case 3 and 4 as $Outbook$.
In this way, we can decode the encoded path information by looking up those two coding books.
For example, given the code ``a[b]c'' where $a$, $b$ and $c$ represent binary sequences,  if the previous edge is noon-backbone edge, we first check if the current coding segment represent entrance symbol in $Inbook$. 
If so, we will apply $Outbook$ to decode the subsequent codes. Otherwise, it means the next edge is still non-backbone edge and $Inbook$ is still effective.
Similar operations are also performed for decoding the edge with backbone edge as previous edge.

Given this, the remaining problem is the estimation of frequencies of entrance and exit symbols since this is the most critical parameter for any coding scheme utilizing information theory (such as Huffman Coding).
Recall that, only case 1 and case 3 cause the using of entrance and exit symbols in the coding scheme.
To address this issue, we use the number of shortest paths passing through consecutive segment $(e_1 \rightarrow e_2)$ as the frequency of entrance symbol ``['', such that $e_1$ and $e_2$ are non-backbone edge and backbone edge, respectively.
Likewise, on the basis of case 3, the number of shortest paths passing through consecutive segment $(e_1 \rightarrow e_2)$ as the frequency of exit symbol ``]'', where $e_1$ and $e_2$ are backbone edge and non-backbone edge, respectively.
In this way, $Inbook$ and $Outbook$ can be correctly updated for encoding and decoding given a new backbone.


In summary, we alteratively utilize two different coding books to decode the path information with the help of a temporary buffer which memorizes the type of previous edge.
We refer to this coding scheme as ``Conditional Coding''. 
The elegance of ``Conditional Coding'' is that coding cost saving is easily achieved by separate coding and decoding process is rather simple as only a temporary buffer is needed.
For any coding scheme which considers incorporating both $Inbook$ and $Outbook$ into one coding book, extra coding cost should be required to distinguish the coding of backbone edges in $Outbook$ and non-backbone edges in $Inbook$. 
Note that, as we have mentioned, for the simplicity of computing penalty $\delta_1$ and saving $\delta_2$, we assume the coding of non-backbone edges are kept while only backbone edges are re-encoded.
However, according to our scheme, non-backbone edges also can be re-encoded to save more coding cost.
Of course, much more computational cost is needed for this dynamic update.


\subsection{Graph Enumeration}
\label{enumeration}

Given the ``core'' of backbone, graph enumeration aims to generate all possible connected subgraph induced by $k$ vertices directly and choose the one with maximal value of objective function as final backbone.
That is, we will try to recursively enumerate all the connected $k$ vertices in the second order graph, and each of such subsets corresponds to a unique candidate of backbone.
However, the problem is how can identify those connected subsets of vertices efficiently.
Clearly, it is too computationally expensive to first enumerate all subsets with $k$ vertices and then identify the best one.
Since the ``core'' of backbone is extracted from second order graph, the final backbone with $k$ vertices in second order graph actually is a subgraph with $k$ edges in the original graph.

In the following, we introduce a approach which uncovers all connected subgraph induced by $k$ vertices. Generally speaking, this algorithm is done in two steps.
In the first step, it tries to find a new connected subgraph with $k$ vertices. Then in the second step, it tries to quickly evaluate the subgraph with regard to objective function.
Algorithm \ref{alg:enumeration} provides the outline of our approach.

\input{Figures/Enum.tex}

To begin with, set $P$ and set $Ex$ are set to be empty and set $N$ is all vertices in $G^\prime$.
Algorithm \ref{alg:enumeration} first check whether the set $P$ which indicates the set of connected vertices in $G^\prime$ reaches the required size (line 1).
If so, its corresponding cost with regard to objective function is evaluated and is compared with existing maximal cost value to decide if better solution has been found (line 2 to 6).
Otherwise, it tries to form new sets $P$ by adding vertex $e$, and set $N$ and $Ex$ by removing all vertices not connected to vertex $e$.
The algorithm continues searching with new sets in a recursive fashion (line 10).
After return, the processed vertex $e$ is removed from candidate set $N$ and put into exclusive set $Ex$ (line 11 to 12).
In this way, the connected subgraph with $k$ vertices with maximal value of objective function is found and returned as backbone. 

==> Related.tex <==
\section{Related Work}
\label{related}

Our problem is highly related to the classical problems so-called maximum-weight connected graph problem (MCG), maximum
edge-weight connected graph problem (MECG) and their variants with some constraints in the field of graph theory. The
problem of maximum-weight connected graph is to find a connected subgraph with k vertices which maximize the sum of
their weights in a vertex-weight graph. It is NP-hard in general, and polynomial solutions utilizing dynamic
programming are available for some special graphs such as tree and layered graphs \cite{Lee96}. In \cite{Ideker02},
Ideker et. al. proved its NP-hardness by the means of reducing minimum set cover problem. Most of work studied the
special case of maximum-weight connected graph problem: the constrained MCG (CMCG), such that a predetermined vertex
should be included in the resulting graph. Lee and Dooly took the CMCG as network flow optimization problem and
formulated it as a linear programming problem in \cite{Lee96}. For general graph, they also introduced a exact
algorithm using Balas additive method with an imbedded connectivity test, and a heuristic algorithm for CMCG in the
paper. Later, Lee and Dolly \cite{Lee98} discussed a class of decomposition algorithms for MCG. The basic idea of those
approaches is to decompose the MCG into several small CMCGs by adding one vertex each time. As the performance is
significantly affected by the ordering of adding vertices, Yamamoto et. al. \cite{Yamamoto09} proposed a new heuristic
based on betweenness centrality to order the vertices, and show their algorithm tend to reduce the number of decomposed
subgraph which eventually leads to the improvement of efficiency. On the other hand, maximum edge-weight connected
graph problem (MECG) tries to find a connected subgraph with $k$ edges which maximize the sum of their edge weights in
a edge-weight graph. Clearly, the only different thing compared with MCG is the goal of maximizing the sum of edge
weights instead of vertex weights. Similarly to MCG, Li et. al. \cite{Li09} studied the special case of maximum
edge-weight connected graph problem (CMECG): constrained MECG with k edges (k-CMECG), such that k given edges should be
included in resulting solution. A exact solution borrowing idea from \cite{Lee96} is proposed for 1-CMECG and a
heuristic algorithm is presented for $k$-CMECG. Typically, those works are also related to $k$-MST problem
\cite{Garg96,Blum96,Awerbuch95} and optimal subgraph extraction problems considering connectivity
\cite{Gabow08,Cheriyan02}.


%Our problem is different from MCG and MECG from two points. First, our problem is more general since we work on a graph
%with weights on both vertices and edges. Therefore, MCG and MECG can be viewed as the special cases of our problem if
%the edge weights or vertices weights are ignored, respectively. Given this, the NP-hardness of our problem is easy to
%obtain. Then, according to the aforementioned objective function, there is a linear relationship between the sum of
%edge weight and the sum of vertex weight. That is, we want to find a subgraph such that the sum of edge weight is
%maximized and the sum of vertex weight is minimized. Clearly, the resulting subgraph should be a subgraph induced by
%its vertex set. Since there is a trade-off between the subgraph size (the number of vertices in the subgraph) and the
%value of objective function, we can not constrain the size of vertices or edges in advance which appears in MCG and
%MECG. Our problem seems harder than classical MCG and MECG, and existing approaches are not directly applicable.


==> Undirected.tex <==
\section{Algorithm for Undirected Graph}
\label{undirected}

In this section, we discuss the backbone discovery problem in undirected graph.
Unlike directed graph which the incoming edges are different from outgoing edges, the rows and the columns in the probability distribution table (as
shown in Figure \ref{bicl}) are the same.
In other words, we have to consider rows and columns simultaneously in the process of extracting backbone edges.
If we directly apply the method for directed graph, the inconsistency of clustering results on those edges with respect to each vertex is a big problem.
For example, given the edge $e_i$ incidents to two endpoints $v_1$ and $v_2$, $e_i$ could be classified as backbone edge if it is viewed as the incoming edge of $v_1$.
However, it is also possible to be labeled as non-backbone edge if $e_i$ is taken as the incoming edge of $v_2$.
In the following, we will utilize an simultaneous biclustering scheme to solve this consistency problem.


In the undirected graph, backbone is discovered in two steps.
To begin with, we view the undirected graph as bi-directed graph and apply the same biclustering algorithm to decompose the incident edges of each vertex into two sets,
and choose the edge set with larger row sums in probability distribution table as backbone edges.
Given this, a novel search procedure including two steps is employed to iteratively refine the backbone until no improvement can be achieved.
In the first step, we use a growing heuristic to extract a connected graph with $k$ vertices.
In the second step, for each pair of connected vertices, we show the consistent backbone edge assignment problem is a biclustering problem,
and thus can be solved by a variant of k-means.
Next, we describe these two steps of iterative refinement procedure in detail.


\subsection{Connected Subgraph with $k$ vertices}

In this step, we assume ``backbone graph'' is obtained by the approach introduced in Section \ref{bediscovery} and try to find a connected subgraph with $k$ vertices.
Since the weight of each vertex is local optimal value, the sum of vertex weights in this connected subgraph is the upper bound of its real value with regard to objective function.
Larger the sum of vertex weight is, more possible real value of objective function can be achieved.
Thus, we actually try to find a connected subgraph with $k$ vertices and large sum of vertex weight.
Of course, we can apply the heuristic algorithm $DEP\_HEU$ introduced in \cite{Lee96} to extract a maximum weight connected subgraph with $k$ vertices.
However, taking the practical issue with respect to its time complexity into consideration, our entire backbone discovery procedure will work in a iterative fashion
and the approach for extracting connected subgraph with $k$ vertices will be invoked several times.
A more efficient heuristic algorithm is much more helpful to reduce the time complexity.
Here, a efficient growing procedure is proposed to find a connected subgraph with $k$ vertices.
The sketch of growing procedure is outlined in Algorithm \ref{alg:expand}.

\input{Figures/DFSExp.tex}

We expand the connected subgraph in recursive way.
For current connected subgraph $G_0$, we pick the vertex $u$ with maximal weight which incident to $G_0$ and is not included in $G_0$
and add into $G_0$.
All relevant edges connecting $u$ and $G_0$ are also added.
Then, the number of vertices to be added is decreased by one.
We recursively apply this growing rule until $k$ vertices are contained in $G_0$.
Clearly, since each time we always select the best vertex incident to existing connected subgraph, the property of connectivity is guaranteed.



\subsection{Edge Refinement}

As mentioned in the beginning of section, the edges in the extracted connected subgraph $G_0$ with $k$ vertices are collected locally and are possible to be inconsistent regarding biclustering.
To address this issue, we put forward a generalized k-means to determine the existence of each edge in $G_0$ in an iterative manner.
We also prove that this procedure is guaranteed to converge in a finite steps.
Specially, as we know, each edge is relevant to two endpoints and their corresponding probability distribution tables.
If we want to determine if this edge should be backbone or non-backbone, these two probability distribution table should be considered simultaneously.
Recall that our goal is to minimize the sum of objective function (i.e. Eq. \ref{funcF}).
Therefore, we only need to check whether the movement for each edge from backbone to non-backbone can result in the improvement of the sum of objective functions on two endpoints.
If so, this edges is considered as non-backbone edge and is removed from $G_0$, otherwise, we keep it.
Since we always improve the sum of two objective function for each movement while do not change others, the sum of values of all objective function is eventually improved.

Formally, assuming two probability distribution table related to two endpoints of one edge $(v_s,v_t)$ are $D_s$ and $D_t$,
the objective function for edge $e$ combines the objective function of two endpoints, that is,
\beqnarr
\label{undirectedobj}
F^\prime = F^\prime(D_1) + F^\prime(D_2) \nonumber \\
 = \sum_{e_j \in nei(v_s)} [(\sum_{e_i \in B_s} N_{ij} \log \frac{p(e_j|e_i)}{p(e_j|B_s)} + \sum_{e_i \in \bar{B}_s} N_{ij} \log \frac{p(e_j|e_i)}{p(e_j|\bar{B}_s)})] \nonumber \\
        + \sum_{e_j \in nei(v_t)}[(\sum_{e_i \in B_t} N_{ij} \log \frac{p(e_j|e_i)}{p(e_j|B_t)} + \sum_{e_i \in \bar{B}_t} N_{ij} \log \frac{p(e_j|e_i)}{p(e_j|\bar{B}_t)})]
\eeqnarr
where $nei(v)$ is the set of edges incident to vertex $v$.
Likewise, applying Lagrange multiplier method, we have
\[ p(e_j|B_s) = \frac{\sum_{e_j \in B_s} N_{ij}}{\sum_{e_i \in nei(s), e_j \in B_s} N_{ij}}  \]
\[p(e_j|\bar{B}_s) = \frac{\sum_{e_j \in \bar{B}_s} N_{ij}}{\sum_{e_i \in nei(s), e_j \in \bar{B}_s} N_{ij}} \]
The value of $p(e_j|B_t)$ and $p(e_j|\bar{B}_t)$ can be obtained similarly.
Given this, we want to determine the cluster membership of edge $e=(v_s,v_t)$ on objective function Eq. \ref{undirectedobj}.

We first describe our generalized k-means in Algorithm \ref{alg:gen2means}, and then formally prove its property of convergence.
The basic idea is to update the cluster membership of each edge based on the integrated improvement from $D_s$
and $D_t$ in a iterative fashion.
Given centroids of two clusters in both probability distribution table,
we assign each edge to the cluster with the smallest sum of two distances to their corresponding centroids at $t$-th iteration, such that
$e_i=(v_s,v_t)$ is non-backbone edge if and only
{\small
\beqnarr
\label{dist}
\sum_{e_j \in nei(v_s)}  N_{ij} \log \frac{p(e_j|e_i)}{p(e_j|B_s)} + \sum_{e_j \in nei(v_t)} N_{ij} \log \frac{p(e_j|e_i)}{p(e_j|B_t)} \nonumber \\
\geq \sum_{e_j \in nei(v_s)} N_{ij} \log \frac{p(e_j|e_i)}{p(e_j|\bar{B}_s)} + \sum_{e_j \in nei(v_t)} N_{ij} \log \frac{p(e_j|e_i)}{p(e_j|\bar{B}_t)}
\eeqnarr
}

\input{Figures/Gen2Means.tex}

In the following, we prove that the value of sum of objective function $F^\prime$ is guaranteed to converge to a local minimum.

\blemma{\bf (Convergence Property)}
\label{converge}
The value of function $F^\prime$ in Eq. \ref{undirectedobj} converges to a local optimum
as we iteratively update membership of edge $e$ in Algorithm \ref{alg:gen2means}.
\elemma
To facilitate the proof, we also consider the edge $e$ which has two endpoints $v_s$ and $v_t$, and their corresponding probability distribution table $D_s$ and $D_t$.
Also, let ${F^\prime}^{(k)}$ be the value of objective function at $k$-th iteration, $c^{(k)}_s(B)$ and $c^{(k)}_s(\bar{B})$ be the centroids of backbone and non-backbone edge set in $D_s$ at $k$-th iteration.
Likewise, we define $c^{(k)}_t(B)$ and $c^{(k)}_t(\bar{B})$ for the centroids in $D_t$.
We denote $dist_{D_s}(e, c)$ and $dist_{D_t}(e,c)$ as the distance between edge $e$ and centroid $c$ in $D_s$ and $D_t$, respectively.
Assume that the algorithm is processing at $k$-th iteration to check the movement of edge $e$.
In the first step for assigning cluster membership, edge $e$ is assigned
to the closest cluster with minimal value of $dist_{D_s}(e, c^{k-1}_s(r))+dist_{D_t}(e,c^{k-1}_t(r))$ where $r=B$ or $\bar{B}$.
On the other hand, we know that the objective function is the sum of distance between each edge and the centroids of cluster to which it belongs.
Therefore, we guarantee that ${F^\prime}^{(t)} \le {F^\prime}^{(t-1)}$, because
{\small
\beqnarr
{F^\prime}^{(t)} - {F^\prime}^{(t-1)} = min\{dist_{D_s}(e, c^{k-1}_s(r))+dist_{D_t}(e,c^{k-1}_t(r)), r=B \mbox{ or } \bar{B}\} \nonumber \\
    - dist_{D_s}(e, c^{k-1}_s(r^\prime))+dist_{D_t}(e,c^{k-1}_t(r^\prime))\le 0
\eeqnarr
}
where $r^\prime$ is the cluster membership of edge $e$ at $(k-1)$-th iteration

For the second step of individually updating centroids, since the new centroids are the optimal center to minimize $F^\prime(D)$ and $F^\prime(D^T)$,
the updated value of objective function ${F^\prime_{new}}^{(k)}$ with new centroids has
{\scriptsize
\beqnarr
{F^\prime_{new}}^{(k)} = {F^\prime_{new}}^{(k)}(D_s) + {F^\prime_{new}}^{(k)}(D_t) \leq {F^\prime}^{(k)}(D_s) + {F^\prime}^{(k)}(D_t) = {F^\prime}^{(k)} \nonumber
\eeqnarr
}
The equality occurs only if this is the last iteration of algorithm.
Therefore, during the process of updating cluster membership of edge $e$, the value of objective function $F^\prime$ is monotonically decreased and eventually converge to a local optimum.
\eproof.


\subsection{Overall Algorithm}

The overall procedure to discover backbone in directed graph is sketched in Algorithm \ref{alg:iterativealg}.
The basic idea is to make full use of recently best result as lower bound to reduce the subsequent search space.
We start with invoking procedure $Expand$ to extract a connected subgraph with $k$ vertices (Line 3).
Then, we compute its sum of vertex weight which is optimized locally for the upper bound (Line 4).
In the edge refinement step (Line 5), generalized k-means is called to determine if each edge is backbone edge and corresponding values of objective function are also updated.
Follow that, we check if the upper bound of $G_0$ is less than best result (i.e., $w_L$) so far.
If not, the procedure is terminated. Otherwise, we continue to update the lower bound if new $w$ is greater than $w_L$.
Finally, we randomly kick out one vertex which is in $G_0$ from $G_c$.
We repeat these steps until the size of remaining graph is too small.
The best result is considered as the final backbone.


\input{Figures/IterDis.tex}

We analyze the complexity in the following.
The preprocessing step is the same with the one in directed graph, which takes $O(|V| (|V|+|E|))$ time.
In the second step of backbone edge discovery, $O(K |E|)$ time is needed, since for each vertex, it takes $O(K |nei(v)|)$ to perform biclustering,
where $K = max(K^\prime)$ and $K^\prime$ is the number of iteration for each vertex.
In Algorithm \ref{alg:iterativealg}, we assume $K_0$ iterations are needed to terminate the procedure.
For each iteration, procedure $Expand$ takes at most $O(|V|)$ time, and procedure $Generalized2Means$ takes at most $O(r^3 K_1)$ time where
$r$ is the number of vertices in backbone, $K_1 $ is the number of iteration in Algorithm \ref{alg:gen2means}.
Putting all together, it takes $O(K_0 (|V|+r^3 K_1))$ time to complete second step.
Overall, the time complexity of backbone discovery scheme on directed graph is $O(|V||E|+K|E|+K_0(|V|+r^3 K_1 ))$.




\comment{
\subsection{Backbone Edge Discovery}

We address the first subproblem in this section.
Since $p(e_j|e_i) \neq p(e_i|e_j)$, the probability distribution table $D$ of each vertex is not symmetric matrix. To
gain better understanding of the problem, we substitute the one probability table $D$ with two tables $D$ and its
transpose matrix $D^T$. Then, the problem is transformed to perform biclustering simultaneously on the rows of both $D$
and $D^T$. The global objective function combines the objective function regards $D$ and $D^T$: \beqnarr
\label{undirectedobj}
F^\prime = F^\prime(D) + F^\prime(D^T) \nonumber \\
 = \sum_{e_j \in nei(v)} [(\sum_{e_i \in B_v} N_{ij} \log \frac{p(e_j|e_i)}{p(e_j|B_v)} + \sum_{e_i \in \bar{B}_v} N_{ij} \log \frac{p(e_j|e_i)}{p(e_j|\bar{B}_v)}) \nonumber \\
        + (\sum_{e_i \in B_v} N_{ij} \log \frac{p(e_i|e_j)}{p(e_j|B_v)^\prime} + \sum_{e_i \in \bar{B}_v} N_{ij} \log \frac{p(e_i|e_j)}{p(e_j|\bar{B}_v)^\prime})]
\eeqnarr where $nei(v)$ is the set of edges incident to vertex $v$, $p(e_j|B_v)^\prime$ and $p(e_j|\bar{B}_v)^\prime$
are the cluster ``centers'' in $D^T$. Likewise, applying Lagrange multiplier method, we have
\[ p(e_j|B_v)^\prime = \frac{\sum_{e_j \in B_v} N_{ij}}{\sum_{e_i \in nei(v), e_j \in B_v} N_{ij}}  \]
\[p(e_j|\bar{B}_v)^\prime = \frac{\sum_{e_j \in \bar{B}_v} N_{ij}}{\sum_{e_i \in nei(v), e_j \in \bar{B}_v} N_{ij}} \]

To solve the problem, we introduce a clustering scheme borrowing idea from k-means to bipartition $D$ and $D^T$ at the
same time. The basic idea is to update the cluster membership of each edge based on the integrated improvement from $D$
and $D^T$ in a iterative fashion. Given centroids of two clusters, we assign each edge to the cluster with the smallest
sum of distances to its centroid at $t$-th iteration, such that
{\small
\beqnarr \label{dist}
S^{(t)}_k = \{ e_i : \sum_{e_j \in nei(v)} ( N_{ij} \log \frac{p(e_j|e_i)}{p^{(t)}_k(e_j|B_v)} +  N_{ij} \log \frac{p(e_i|e_j)}{p^{(t)}_k(e_j|B_v)^\prime}) \nonumber \\
 \leq \sum_{e_j \in nei(v)} ( N_{ij} \log \frac{p(e_j|e_i)}{p^{(t)}_m (e_j|B_v)} + N_{ij} \log \frac{p(e_i|e_j)}{p^{(t)}_m(e_j|B_v)^\prime} ) \nonumber \\
 \mbox{ for all m = 0 or 1} \}
\eeqnarr
}
We outline the clustering scheme in Algorithm \ref{alg:biclustering}. The key building block of our procedure
is the employment of cluster assignment and centroid calculation to achieve local optimum in a finite steps (as
formally stated in Lemma \ref{converge}).

\input{Figures/Bicluster.tex}

\blemma{\bf (Convergence Property)} \label{converge} The value of function $F^\prime$ in Eq. \ref{undirectedobj}
converges to a local optimum in a finite steps as we iteratively invoke two steps in Algorithm \ref{alg:biclustering}.
\elemma

\bproof Let $W=\{w_i, 0 \leq i < |nei(v)|\}$ be the indicator vector for the clustering of edges incident to vertex
$v$. Since it is biclustering problem, we use binary value to determine if one edge belong to one cluster, such that if
$e_i$ belongs to cluster $B_v$, $w_i=1$; otherwise, $w_i = 0$. Clearly, each binary sequence with length $|nei(v)|$
corresponds to one feasible cluster assignment $W$. We note that there are only a finite number of feasible assignments
(i.e., $2^{|nei(v)|}$). Then, we show that each feasible assignment appears at most once by the Algorithm
\ref{alg:biclustering}.

First, we demonstrate that the value of $F^\prime$ is monotonically decrease as the algorithm processing. For
simplicity, let ${F^\prime}^{(t)}$ be the value of objective function at $t$-th iteration, $c^t_k$ be the centroid of
cluster $k$ (i.e., $k=0$ or $1$ at $t$-th iteration). We denote $dist_D(e_i, c)$ and $dist_{D^T}(e_i,c)$ as the distance
between edge $e_i$ and centroid $c$ in probability distribution table $D$ and $D^T$, respectively. Assume that the
algorithm is processing at $t$-th iteration. In the first step for assigning cluster membership, each edge is assigned
to the closest cluster with minimal value of $dist_D(e_i, c^{t-1}_k(D))+dist_{D^T}(e_i,c^{t-1}_k(D^T))$. In other
words, we guarantee that ${F^\prime}^{(t)} \leq {F^\prime}^{(t-1)}$. For the second step of individually updating
centroids, since the new centroids are the optimal center to minimize $F^\prime(D)$ and $F^\prime(D^T)$, we note that
updated value of objective function ${F^\prime_{new}}^{(t)}$ with new centroids
{\scriptsize
\beqnarr
{F^\prime_{new}}^{(t)} = {F^\prime_{new}}^{(t)}(D) + {F^\prime_{new}}^{(t)}(D^T) \leq {F^\prime}^{(t)}(D) + {F^\prime}^{(t)}(D^T) = {F^\prime}^{(t)} \nonumber
\eeqnarr
}
The equality between old and new value of $F^\prime$ occurs only if this is the last iteration of algorithm.
Therefore, during the process of algorithm, the value of objective function is strictly decreased.
Assuming one
feasible assignment appears two times (e.g., $t_1$-th iteration and $t_2$-th iteration) during the process, that means
the value of objective function between $t_1$-th iteration and $t_2$-th iteration are the same, which leads to a
contradiction with our aforementioned conclusion. Hence the convergence property holds in Algorithm \ref{alg:biclustering}.
\eproof


\subsection{Iterative Algorithm for Connected Subgraph with $r$ vertices}
\label{iterativealg}

Given the extracted backbone edges and its corresponding value of objective function,
the remaining issue is to identify a connected subgraph with $r$ vertices which maximizes the global objective function in Eq. \ref{bbmdl}.
To facilitate the following discussion, each vertex is assigned the weight as the value of objective function.
As we have mentioned, we cannot apply the algorithm used for directed graph here, because backbone edges are extracted with regard to each vertex indivually
which probably leads to inconsistency.

In this section, we put forward a novel scheme based on sampling technique to solve it.
The basic idea is to make full use of recently best result as lower bound to reduce the subsequent search space.
Specially, we begin with a ``good'' starting point such that a connected subgraph with $r$ vertices and large sum of their vertices weight.
This can be achieved by traversing the graph from different starting points with the rule that the vertex with larger weight has higher priority to be visited.
Since the vertex weight is gained without considering the inconsistency from its neighbors, it is definitely greater than the value of objective function which takes others into consideration.
Therefore, the sum of vertex weight in this connected subgraph can be viewed as the upper bound of the value of objective function it can achieve.
Supposing that this connected subgraph is the backbone, we can calculate the real value of objective function by invoking biclustering on each vertex until the clustering results are consistent between each pair of connected vertices.
Note that, we just consider the edges in backbone graph.
This value is taken as the lower bound, because no matter what happen in the following iteration, our final result cannot be worse than this one.
In the next iteration, we randomly remove one vertex including in the current backbone from the network.
Then, we perform the same procedure to seek a new backbone.
We repeat this procedure until the upper bound of current connected subgraph is not better than the lower bound of backbone so far.
The backbone corresponding to the lower bound is considered as the final result.
The entire algorithm is illustrated in Algorithm \ref{alg:iterativealg}.



\input{Figures/IterDis.tex}


We analyze the complexity in the following.
The preprocessing step is the same with the one in directed graph, which takes $O(|V| TC(G))$ time.
In the second step of backbone edge discovery, $O(K |E|)$ time is needed, since for each vertex, it takes $O(K |nei(v)|)$ to perform simultaneous biclustering,
where $K = max(K^\prime)$ and $K^\prime$ is the number of iteration for each vertex.
In Algorithm \ref{alg:iterativealg}, we assume $k_0$ iterations are needed to terminate the procedure.
For each iteration, procedure $Expand$ takes at most $O(|V|)$ time, and \textcolor{red}{the time for updating objective function assuming backbone is given is $T$???????}.
Putting all together, it takes $O(k_0 (|V|+T))$ time to complete second step.
Overall, the time complexity of backbone discovery scheme on directed graph is $O(K|E|+K_0(|V|+T))$.
}

